Leveraging Meta-path Contexts for Classification in Heterogeneous Information Networks

A heterogeneous information network (HIN) has as vertices objects of different types and as edges the relations between objects, which are also of various types. We study the problem of classifying objects in HINs. Most existing methods perform poorly when given scarce labeled objects as training sets, and methods that improve classification accuracy under such scenarios are often computationally expensive. To address these problems, we propose ConCH, a graph neural network model. ConCH formulates the classification problem as a multi-task learning problem that combines semi-supervised learning with self-supervised learning to learn from both labeled and unlabeled data. ConCH employs meta-paths, which are sequences of object types that capture semantic relationships between objects. ConCH co-derives object embeddings and context embeddings via graph convolution. It also uses the attention mechanism to fuse such embeddings. We conduct extensive experiments to evaluate the performance of ConCH against other 15 classification methods. Our results show that ConCH is an effective and efficient method for HIN classification.

==> tex/algorithm_report.tex <==
\section{Algorithm}
\label{sec:algorithm}

In this section we describe our ROSC algorithm. Figure~\ref{figure:flow_graph}(c) shows a 
flow diagram of ROSC. ROSC follows the basic pipeline of spectral clustering except that
it generates a coefficient matrix $Z$ 
%(shown in the red box of the diagram) 
and feeds it
 into the clustering pipeline in place of
the similarity matrix $S$. 
The objective is to find a  $Z$ that possesses  grouping effect. 
To achieve that, ROSC uses PI to obtain {\pev}s from which a basic $Z$ is derived.
Next, it generates the TKNN graph with which $Z$ is rectified. 
In the following, we discuss how $Z$ is derived from the {\pev}s, define the TKNN graph,
describe the rectification process, 
and prove that the resulting $Z$ has the desired grouping effect. 

%
%In this section, we propose a \textbf{RO}bust \textbf{S}pectral \textbf{C}lustering method ROSC. 
%Instead of directly performing spectral clustering on the given similarity matrix, 
%it constructs a new matrix that reserves the efficacy of effective similarities 
%and rectifies ineffective ones in the raw similarity matrix.
%The new matrix will lead to a more robust spectral clustering.

\comment{
\subsection{Model overview}
The overall framework of ROSC is summarized as follows.

First, generate a set of pseudo-eigenvectors.
Since the standard spectral clustering methods using only the dominant eigenvectors may fail 
in the data containing multi-scale clusters,
we generate a set of pseudo-eigenvectors to fuse more useful cluster-separation information.

Second, rectify the given similarity matrix.
The failure of spectral clustering on multi-scale data originates from the inaccurate similarity matrix.
Therefore, we rectify the matrix and aim to achieve a new one
that can more accurately reflect the true similarities between objects.
%This is a major problem to be addressed.

Third, perform spectral clustering.
After rectification, the new similarity matrix will be more accurate and it will be safer to perform spectral clustering. 

These three steps will lead to robust clustering results and next we introduce each step in detail.
}

\subsection*{Pseudo-Eigenvectors}
\label{sec:sec:pseudo}
Given a similarity matrix $S$, we normalize it and apply PI to obtain {\pev}s.
%When dealing with multi-scale data,
%spectral clustering
%using only the top-$k$ eigenvectors may fail while some other eigenvectors may be useful~\cite{lin2010power}.
%Therefore, it is necessary to fuse the discriminative cluster-separation information in all eigenvectors
%and PI provides such fusion by returning a pseudo-eigenvector.
%However, when the number of clusters is large,
%a single pseudo-eigenvector is insufficient due to the cluster-collision problem. 
%%Since PI returns a pseudo-eigenvector that is a combination of all the eigenvectors,
Similar to~\cite{ye2016fuse},
we run PI multiple times with different random initial vectors to generate a set of {\pev}s, 
which maps each object into a low dimensional embedding.
Note that small {\ev}s are {\it shrunk} by PI~\cite{lin2010power}.
%\footnote{From Equation~\ref{eq:pi}, we see that the $i$-th 
%largest \ev\ is 
%shrunk at a rate of $\lambda_i/\lambda_1$ per iteration.}.
To alleviate the shrinkage of small {\ev}s,
we follow the approach of~\cite{huang2014diverse}
and gradually decrease the number of iterations executed in PI as more {\pev}s are obtained. 

Since the {\pev}s approximate the most dominant {\ev}, they could be similar. 
To reduce this redundancy,
whitening~\cite{kessy2017optimal} is used to make the pseudo-eigenvectors uncorrelated.
Moreover, noise in the {\pev}s are reduced 
by a rectification process, which will be discussed later.

\comment{
First, we generate a set of pseudo-eigenvectors using different random vectors $\bm{v}_0$.
From Eq.~\ref{eq:v0}, $\bm{v}_0$ can be represented by the subspace spanned by all the eigenvectors.
Suppose $\bm{e}_i$ is an informative eigenvector with a relatively small eigenvalue $\lambda_i$.
Given a $\bm{v}_0$, if it has a dominant component in the direction of $\bm{e}_i$, 
i.e., the associated coefficient $c_i$ is large, 
with an appropriate number of iterations, $c_i\lambda_i^t\approx c_2\lambda_2^t$,
the effect of $\bm{e}_i$ will be finally retained in the pseudo-eigenvector.
Therefore, multiple pseudo-eigenvectors generated by different $\bm{v}_0$
may increase the chance to hold all the informative eigenvectors.

Second, we can control the number of iterations in PI.
In PIC, the \emph{velocity} and \emph{acceleration} at the $t$-th iteration are respectively defined as
$\bm{\delta}_t = \bm{v}_t - \bm{v}_{t-1}$ and $\bm{\epsilon}_t = \bm{\delta}_t-\bm{\delta}_{t-1}$.
A threshold $\epsilon$ is introduced to measure the acceleration change in two consecutive iterations 
and stop PI when $|\bm{\epsilon}_t-\bm{\epsilon}_{t-1}|<\epsilon$.
However,
since the effect of eigenvectors corresponding to smaller eigenvalues will shrink as $t$ increases,
we can decrease the number of iterations by gradually increasing the $\epsilon$ value,
which provides another way to keep useful information in ``less important'' eigenvectors. 
}

\subsection*{Transitive {\it K} Nearest Neighbor (TKNN) Graph}

%\begin{figure}
%    \centering
%        \includegraphics[width = 0.8\linewidth]{figure/example1.eps}
%        \caption{An toy example}
%        \label{figure:example1}
%\end{figure}

%The \emph{$K$ nearest neighbor} (KNN) graph is generally used to depict the most adjacent relations between objects,
%in which the linked objects are generally assumed to share common characteristics.
%Given a set of objects $\mathcal{X} = \{\bm{x}_1,\bm{x}_2,...,\bm{x}_n\}$,
%the KNN graph $G_{K} = (V, E)$ is a graph with $V = \mathcal{X}$ and $E = \{e_{ij}\}$.
%%An edge $e_{ij}$ between $\bm{x}_i$ and $\bm{x}_j$ indicates
%%$x_j \in N_K(\bm{x}_i)$ or $x_i \in N_K(\bm{x}_j)$,
%%where $N_K(\bm{x}_i)$ denotes the set of $K$ nearest neighbors of $\bm{x}_i$.
%%at least one of the two end nodes is in the $K$ nearest neighborhood of the other.
%%However, the $K$ nearest neighborhood relation is not symmetric,
%%i.e., $x_j \in N_K(\bm{x}_i)$ is inequivalent to $x_i \in N_K(\bm{x}_j)$, 
%Some previous work~\cite{yin2016laplacian} simply considers $e_{ij}$
%exists when $\bmx_j \in N_K(\bmx_i)$ or $x_i \in N_K(\bmx_j)$,
%where $N_K(\bmx_i)$ denotes the set of $K$ nearest neighbors of $\bmx_i$.
%However,
%in the case of data containing multi-scale clusters,
%such definition may lead to an edge between
%two objects in different clusters.
%Fig.~\ref{figure:example1} shows an toy example which consists of two multi-scale clusters
%marked by ``$\times$" and ``$+$" respectively.
%For object $\bmx_1$,
%object $\bmx_2$ is its nearest neighbor.
%But for $\bmx_2$, $\bmx_1$ is far away from it.
%In this case, there will be an edge between $\bmx_1$ and $\bmx_2$ in the traditional KNN graph.
%However, since $\bmx_1$ and $\bmx_2$ belong to different clusters,
%they should not be connected.

Our objective is to capture the high correlations between objects that belong to the same cluster even 
 though the objects could be located at distant far ends of a cluster. 
 These correlations are expressed via a TKNN graph, which is used to 
 regularize the coefficient matrix $Z$.

\begin{definition}
\label{def:nei_relation}
\textbf{(Mutual  $K$-nearest neighbors)}
Let $N_K(x)$ be the set of $K$ nearest neighbors of an object $x$.
Two objects $x_i$ and $x_j$ are said to be mutual $K$-nearest neighbors of each other,
denoted by $x_i \sim x_j$, 
iff $x_i \in N_K(x_j)$ and $x_j \in N_K(x_i)$.
\hfill$\Box$
\end{definition}

%In the case of multi-scale data,
%the KNN graph is sometimes insufficient to reflect whether two objects belong to the same cluster or not.
%For example, objects $\bmx_2$ and $\bmx_3$ in Fig.~\ref{figure:example1} belong to the same cluster, 
%but they are both far away from each other.
%%objects $x_1$ and $x_2$ are in different clusters despite their closeness.
%To construct an effective KNN graph, $\bmx_2$ and $\bmx_3$
%are expected to be linked.
%Therefore,
%the reachability between two objects is introduced.

\begin{definition}
\label{def:reachability}
\textbf{(Reachability)}
Two objects $x_i$ and $x_j$ are said to be reachable from each other
if there exists a sequence of $h \geq 2$ objects 
 $\{x_i = x_{a_1}, \ldots, x_{a_h} = x_j\}$ such that
 $x_{a_r} \sim x_{a_{r+1}}$ for $1 \leq r < h$.
 \hfill$\Box$
\end{definition}

\begin{definition}
\label{def:trans_relation}
\textbf{(Transitive $K$-nearest neighbor (TKNN) graph)}
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
the TKNN graph $\mathcal{G}_K = (\mathcal{X},\mathcal{E})$
is an undirected graph
where $\mathcal{X}$ is the set of vertices and $\mathcal{E}$ is the set of edges.
Specifically, the edge ($x_i$, $x_j$) $\in \mathcal{E}$
iff $x_i$ and $x_j$ are reachable from each other.
We represent the TKNN graph by an $n \times n$ {\it reachability matrix}
$\mathcal{W}$ 
whose ($i$,$j$)-entry $\mathcal{W}_{ij} = 1$ if ($x_i$, $x_j$) $\in \mathcal{E}$; 0 otherwise.
\hfill$\Box$
\end{definition}

%We note that mutual-KNN is a symmetric relation and so is reachability. 

%Compared with the traditional KNN graph, 
%the TKNN graph can more accurately reflect 
%whether two objects belong to the same cluster or not.
%It will be used in the next section to rectify the matrix of similarity between objects.
 
\subsection*{Coefficient Matrix}
%In the case of multi-scale data,
%the distance-based similarity is likely to be ineffective. 
%To improve the clustering performance,
%it is necessary to rectify the matrix.
%The rectification should follow two principles.
%First, for the effective similarities, the efficacy should be reserved.
%Second, for the ineffective ones, the efficacy should be enhanced.
%For example,
%the closeness between objects $\bmx_3$ and $\bmx_4$ in Fig.~\ref{figure:example1}
%leads to a large similarity value.
%Since the two objects are of the same cluster,
%the new value should still be large.
%In comparison, 
%both the similarity between $\bmx_1$ and $\bmx_2$ and the one between $\bmx_2$ and $\bmx_3$
%should be rectified, as these distance-based similarities are ineffective.

%In the multi-scale data,
%different clusters may have different sizes, densities or even geometric structures.
The similarity between two objects describes the degree to which they share common characteristics.
The more similar they are, 
the more likely that one object can be represented by the other. 
Therefore,
to depict the relationships between objects in multi-scale data,
each object is linearly characterized by other objects,
assuming the well-known linear subspace model~\cite{liu2013robust}.

We generate $p$ {\pev}s using PI. 
%just as a non-linear manifold can be locally approximated by linear subspaces.
%First, these vectors, which retain the effects of dominant eigenvectors,
%can certainly retain the original accurate similarities between objects.
%Second, they absorb the cluster-separation information from the seemingly ``less important'' eigenvectors,
%which further provides a reliable source of information to rectify the erroneous similarities.
Let $X\in \mathcal{R}^{p\times n}$ be a matrix whose rows are the {\pev}s.
The $q$-th column of $X$ can be taken as a feature vector $\bmx_q$ of an object $x_q$.
We normalize the column vectors of $X$ such that $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$.
We determine a coefficient matrix $Z \in \mathcal{R}^{n \times n}$ by
\begin{equation}
\label{eq:nonoise}
X = XZ,\;\;\; \text{s.t. } diag(Z) = 0.
\end{equation} 
One can interpret $Z_{ij}$ 
as a value that reflects how well object $x_i$ characterizes object $x_j$.
The constraint $diag(Z) = 0$ avoids the trivial solution of $Z$ equals the identity matrix.
For simplicity, we do not explicitly mention this constraint in the rest of the paper.

As indicated by previous works~\cite{ye2016fuse}, the generated pseudo-eigenvectors are likely to be noise-corrupted.
We thus extend Equation~\ref{eq:nonoise} by introducing a noise matrix $O$, giving:
%However, although the pseudo-eigenvectors inherit useful cluster-separation information,
%they may also be contaminated by noise.
%Thus a matrix $O$ is introduced to capture the noise,
\begin{equation}
X = XZ + O.
\label{eq:O}
\end{equation} 
%The TKNN graph conveys information on whether two objects belong to the same cluster or not,

As we have explained, the TKNN graph  conveys useful clustering information, bringing highly
correlated objects that are located at distant far ends of a cluster together.
We thus use the TKNN graph to regularize matrix $Z$.
We derive the following objective function:
%Since our objective is to derive a $Z$ which can better reflect the true similarities between objects,
\comment{
\begin{equation}
%\label{eq:obj}
\min_Z ||O||_F^2+\lambda_1||Z||_F^2 + \lambda_2||Z-\mathcal{W}_K||_F^2,
s.t., X = XZ+O,
\end{equation}
}
%By substituting $O$, we derive
\begin{equation}
\label{eq:obj_constraint}
\min_Z ||X-XZ||_F^2 + \alpha_1 ||Z||_F^2 + \alpha_2 ||Z-\mathcal{W}||_F^2,
\end{equation}
where $\alpha_1 > 0,\alpha_2 \geq 0$ are two 
weighting factors that adjust the relative weights of the three components that constitute
the objective function.
The objective function consists of three terms.
The first term aims to reduce the noise matrix $O$ (see Equation~\ref{eq:O}),
the second term is the Frobenius norm on $Z$, and
%that restricts any item in $Z$ from being dominant.
the third term regularizes $Z$ by the TKNN graph.
%For simplicity, as in~\cite{lu2012robust},
%we remove the constraint and formulate the problem as
%\begin{equation}
%\label{eq:obj}
%\min_Z ||X-XZ||_F^2 + \lambda_1 ||Z||_F^2 + \lambda_2 ||Z-\mathcal{W}_K||_F^2.
%\end{equation}
%$\lambda_1$ and $\lambda_2$ are two parameters to balance the effects of three parts.
A closed-form solution, $Z^*$, to the optimization problem is
\begin{equation}
\label{eq:solution}
Z^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^TX+\alpha_2\mathcal{W}).
\end{equation}

\subsection*{Grouping Effect}
For an object $x_p$, 
let $\bmz_p$ be the $p$-th column of the coefficient matrix $Z$.
We interpret the entries of $\bmz_p$ as the coefficients that express $x_p$ as a linear combinations
of other objects. 
Previous works~\cite{lu2012robust,lu2013correlation,hu2014smooth} have shown that if $Z$ has {\it grouping effect}, then performing spectral 
clustering based on $Z$ would be effective. 
Intuitively, $Z$ has grouping effect if, given two {\it highly correlated} objects $x_i$ and $x_j$,
their characterization of other objects are similar.
Existing works mostly consider {\it high correlation} between objects as {\it high similarity} of their
feature vectors. With ROSC, we consider object similarity in terms of both feature similarity and 
reachability similarity. 
Feature similarity is measured by the objects' feature vectors as given by the columns of matrix $X$.
Reachability similarity is measured by the columns of matrix $\mathcal{W}$, 
each of which shows the reachability of an object to all others. 
Formally,



%It has been shown that the first two terms in the objective function decide the \emph{grouping effect} of $Z$~\cite{lu2012robust}.
%In Problem~\ref{eq:obj}, the first two terms decides whether $Z$ has the grouping effect~\cite{lu2012robust} defined as follows.
%i.e., the more highly correlated two objects are,
%the larger weight one will have in characterizing the other~\cite{lu2012robust}.

\begin{definition}
\label{def:grouping}
\textbf{(Grouping effect)}. 
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
let $\bmw_q$ be the $q$-th column of $\mathcal{W}$. 
Further, let $\xarrow{i}{j}$ denote the condition:
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and 
(2) $\lVert \bmw_i - \bmw_j \rVert_2 \rightarrow 0$.
A Matrix $Z$ is said to have grouping effect
if
\[
\xarrow{i}{j} \Rightarrow |Z_{ip} - Z_{jp}| \rightarrow 0\; \forall 1 \leq p \leq n.
\]
%for an arbitrary object $\bmx$ and its associated coefficient vector $\bm{z}$,
%If $\bmx_i\rightarrow \bmx_j$,
%then $z_{pi}\rightarrow z_{pj}$,
%where $z_{pi}$ and $z_{pj}$ are the $i$th and $j$th entry in $\bm{z}_p$ respectively.
%Then we say the self-representation matrix $Z$
%has the grouping effect.
%\hfill$\Box$
\end{definition}

Our next task is to prove that the optimal solution $Z^*$ (as given in Equation~\ref{eq:solution})
% of Equation~\ref{eq:obj_constraint}
has the grouping effect.
In the following discussion, we use $\bmz_q^*$ to denote the $q$-th column vector of $Z^*$.

\begin{lemma}
\label{lemma1}
Given a set of objects $\mathcal{X}$,
the matrix
$X\in \mathcal{R}^{p\times n}$ that is composed of the {\pev}s as rows,
 the reachability matrix $\mathcal{W}$,
 and the optimal soution $Z^*$ of Equation~\ref{eq:obj_constraint},
\begin{equation}
\label{eq:zi}
Z_{ip}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 \mathcal{W}_{ip}}{\alpha_1+\alpha_2}, \;\;\; \forall 1 \leq i, p \leq n.
\end{equation}
\end{lemma}

\begin{proof}
For $1 \leq p \leq n$,
let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \alpha_1 ||\bm{z}_p||_2^2 + \alpha_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
Since $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have $\frac{\partial{J}}{\partial{Z}_{ip}}|_{\bm{z}_p = \bm{z}_p^*} = 0\; \forall 1\leq i \leq n$.
Hence, $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\alpha_1Z_{ip}^*+2\alpha_2(Z_{ip}^*-\mathcal{W}_{ip}) = 0$,
which induces Equation~\ref{eq:zi}.
\end{proof}

%\begin{lemma}
%\label{lemma1}
%Given a set of objects $X\in \mathcal{R}^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object and $\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bmx_p$.
%Each item $z_{pi}^*$ in the optimal solution $\bm{z}_p^*$ to the problem 
%$\min_{\bm{z}} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$ is
%\begin{equation}
%\label{eq:zi}
%z_{pi}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \lambda_2 w_{pi}}{\lambda_1+\lambda_2},
%\end{equation}
%where $w_{pi} = 1$, if $\bm{x_p}$ and $\bm{x}_i$ are reachable; $0$, otherwise. 
%
%Proof. Let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Since $\bm{z}_p^*$ is the optimal solution, then $\frac{\partial{J}}{\partial{z}_{pi}}|_{\bm{z}_p = \bm{z}_p^*} = 0$.
%Thus we have $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\lambda_1z_{pi}^*+2\lambda_2(z_{pi}^*-w_{pi}) = 0$,
%which induces Eq.~\ref{eq:zi}.
%\end{lemma}

\comment{
Eq.~\ref{eq:zi} calculates the weight of object $\bm{x}_i$ in characterizing $\bm{x}$.
For $w_i$, if $\bm{x}$ and $\bm{x}_i$ are reachable in the TKNN graph, $w_i = 1$; otherwise, $w_i = 0$. 
Eq.~\ref{eq:zi} rectifies the ineffective similarity as follows.
When $\bm{x}$ and $\bm{x_i}$ are far away from each other in the feature space
but reachable in the TKNN graph,
$z_i$ will be increased by $w_i = 1$.
%which rectifies the original incorrect similarity value between them.
Moreover, if $\bm{x}$ and $\bm{x}_i$ are highly correlated,
the first two terms in the problem can decide a large $z_i$,
even in the case that they are unreachable.
%$z_i$ can still keep large with a small $\lambda_2$.
In summary, Eq.~\ref{eq:zi} can not only hold the original accurate similarities but also rectify the incorrect ones.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space but connected in the TKNN graph, 
their similarity will be increased.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space and disconnected in the TKNN graph, 
their similarity will be further decreased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space and connected in the TKNN graph,
their similarity will be further increased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space but disconnected in the TKNN graph,
their similarity will be decreased. In this case,
provided that the raw similarity is effective already,
even though the new value will be decreased,
but it will be still
}

\begin{lemma}
\label{lemma2}
%Given a set of objects $X\in R^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object, 
%$\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bm{x}_p$, and
%$\bm{z}_p^*$ be the optimal solution to the problem 
%$\min_{\bm{z}_p} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Assume all the objects have been normalized.
%For any two objects $\bm{x}_i$ and $\bm{x}_j$,
$\forall 1 \leq i, j, p \leq n$,
\begin{equation}
\label{eq:norm}
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)} + \alpha_2|\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2},
\end{equation}
where $c = \sqrt{1+\alpha_2||\bm{w}_p||_2^2}$ and $r = \bm{x}_i^T\bm{x}_j$.
\end{lemma}

\begin{proof}
From Equation~\ref{eq:zi}, we have 
\begin{equation}
\nonumber
Z_{ip}^*-Z_{jp}^* = \frac{(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 (\mathcal{W}_{ip}-\mathcal{W}_{jp})}{\alpha_1+\alpha_2}.
\end{equation}
That implies 
\begin{small}
\begin{equation}
\label{eq:zizj}
\begin{split}
|Z_{ip}^*-Z_{jp}^*| & \leq \frac{|(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*)| + \alpha_2 |(\mathcal{W}_{ip}-\mathcal{W}_{jp})|}{\alpha_1+\alpha_2}\\
& \leq \frac{||(\bm{x}_i^T - \bm{x}_j^T)||_2||(\bm{x}_p-X\bm{z}_p^*)||_2 + \alpha_2 |(\mathcal{W}_{ip}-\mathcal{W}_{jp})|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
\end{small}

Since the column vectors of $X$ are normalized (i.e., $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$) , we have
$||(\bm{x}_i^T - \bm{x}_j^T)||_2 = \sqrt{2(1-r)}$,
where $r = \bm{x}_i^T\bm{x}_j$.
%measuring the closeness between $\bm{x}_i$ and $\bm{x}_j$ in the feature space.
%As $\bm{z}_p^*$ is the optimal solution, 
As $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have
\begin{equation}
\begin{split}
J(\bm{z}_p^*) & = ||\bm{x}_p-X\bm{z}_p^*||_2^2 + \alpha_1 ||\bm{z}_p^*||_2^2 + \alpha_2 ||\bm{z}_p^*-\bm{w}_p||_2^2 \leq  \\
J(\bm{0}) & = ||\bm{x}_p||_2^2 + \alpha_2 ||\bm{w}_p||_2^2 = 1 + \alpha_2 ||\bm{w}_p||_2^2.
\end{split}
\end{equation}
Hence, $||\bm{x}_p-X\bm{z}_p^*||_2 \leq \sqrt{1 + \alpha_2 ||\bm{w}_p||_2^2} = c$.
Equation~\ref{eq:zizj} can be further simplified as
\begin{equation}
\nonumber
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)}+ \alpha_2 |(\mathcal{W}_{ip}-\mathcal{W}_{jp})|}{\alpha_1+\alpha_2}.
\end{equation}
\end{proof}

\begin{lemma}
Matrix $Z^*$ has grouping effect.
\label{lemma:z-star}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$ such that $\xarrow{i}{j}$,
we have,  %by definition, 
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and (2) $||\bmw_{i}-\bmw_{j}||_2 \rightarrow 0$.
These imply
$r = \bmx_i^T \bmx_j \rightarrow 1$ and  $|\mathcal{W}_{ip}-\mathcal{W}_{jp}| \rightarrow 0$.
Hence, the two terms of the numerator of the R.H.S of Equation~\ref{eq:norm} are close to 0. 
Therefore, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$ and thus $Z^*$ has grouping effect.
\end{proof}

Indeed, Equation~\ref{eq:norm} shows how our algorithm ROSC enhances the effectiveness of 
spectral clustering on multi-scale data. 
Comparing with traditional approaches, which focus on feature similarity, ROSC uses $Z^*$
to integrate feature similarity  ($r$) with
reachability similarity ($|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$).
In particular, two distant objects $x_i$ and $x_j$ of a cluster may not share a strong feature similarity.
This leads to a small $r$ and traditional approaches will likely put them into separate clusters.
On the contrary, ROSC considers the strong reachability of the objects
to derive a small value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$, and thus keeping them in the same cluster.
Moreover, for $x_i$ and $x_j$ that belong to two different dense clusters but happen to be close in 
space (i.e., $x_i$ and $x_j$ have strong feature similarity), 
traditional approaches may inadvertently merge them into the same cluster. 
ROSC, however, would discover their low reachability (via the mutual-KNN relation)
and derive a large value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$.
This regulates matrix $Z^*$ and avoids the incorrect merging.
As we will see in the next section, ROSC's approach 
greatly improves clustering quality and is more robust than other algorithms in handling
multi-scale data.
 
%Lemma~\ref{lemma1} and~\ref{lemma2} prove the grouping effect of $Z^*$ derived by Eq.~\ref{eq:solution}.
%%the weight difference of two objects in characterizing an arbitrary object $\bm{x}$ is bounded.
%Given two objects $\bmx_i$ and $\bmx_j$, if $\bmx_i \rightarrow \bmx_j$, 
%i.e., $\bmx_i^T \bmx_j \rightarrow 1$ and $||w_{pi}-w_{pj}||_2 \rightarrow 0$,
%then $||z_{pi}^*-z_{pj}^*||_2 \rightarrow 0$.
%%which shows the grouping effect of $Z$ derived by Eq.~\ref{eq:solution}.
%%However, in the case of (1) $\bm{x}_i^T\bm{x}_j = 0$ but $w_i=w_j=1$ and 
%%(2) $\bm{x}_i^T\bm{x}_j = 1$ but $||w_i-w_j||_2=1$,
%%$||z_i^*-z_j^*||_2$ can still be small with an appropriate setting on $\lambda_1$ and $\lambda_2$.
%%Further, since $Z$ can not only retain the accurate similarities but also rectify the incorrect ones, 
%%In other words, objects in the same cluster will be better reflected in the rectified matrix.
%%Such grouping effect together with The rectification ability could guarantee a more robust clustering performance.
%We then summarize how the TKNN graph rectifies the raw similarity matrix.
%Given any two objects $\bmx_i$ and $\bmx_j$,
%\begin{enumerate}[label=(\arabic*), leftmargin=*]
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\setlength{\parskip}{0pt}
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be increased.
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be further decreased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be further increased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be decreased.
%\end{enumerate}
%Among the four cases,
%$Z$ reserves the efficacy of effective similarities by (2) and (3)
%while it enhances the efficacy of ineffective similarities by (1) and (4). 
%Thus spectral clustering based on $Z$ will be more robust.

\comment{
\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 0$ but reachable, $S_{ij}$ will be increased.

\noindent{\small$\bullet$}
%For any two objects dissimilar in the feature space and disconnected in the TKNN graph, their similarity will be further decreased.
$\bmx_i^T \bmx_j \rightarrow 0$ and unreachable, $S_{ij}$ will be further decreased.

\noindent{\small$\bullet$}
%For any two objects similar in the feature space and connected in the TKNN graph, their similarity will be further increased.
$\bmx_i^T \bmx_j \rightarrow 1$ and reachable, $S_{ij}$ will be further increased.

\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 1$ but unreachable, $S_{ij}$ will be decreased.
}

\subsection*{ROSC: Robust Spectral Clustering}
%The coefficient matrix $Z$ take advantage of both cluster-separation information in all the eigenvectors
%and the TkNN graph, which not only retains the original accurate similarities but also rectifies the incorrect ones.

We note that the matrix $Z^*$ obtained may be asymmetric and it may contain negative values.
To construct a matrix of object similarity, a common fix~\cite{liu2013robust,lu2012robust} is to 
compute $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$.
After $\tilde{Z}$ is computed, ROSC executes a standard spectral clustering method
(e.g., NCuts) using $\tilde{Z}$ as the similarity matrix in place of $S$.
It can be proved that $|Z^*|$, $|(Z^*)^T|$, and hence $\tilde{Z}$ all have grouping effect.
%Due to space limitations, readers are referred to [XXX] for the proofs. 
Finally, ROSC is summarized in Algorithm~\ref{alg}.


\begin{lemma}
Matrix $|Z^*|$ has grouping effect.
\label{lemma:z-star-abs}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$,
we have 
$\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \leq |Z_{ip}^*-Z_{jp}^*|$.
From Lemma~\ref{lemma:z-star},
$Z^*$ has grouping effect, i.e.,
if $x_i \rightarrow x_j$, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$.
Thus $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and 
$|Z^*|$ has grouping effect.
\end{proof}

\begin{lemma}
\label{lemma3}
$(Z^*)^T$ and $|(Z^*)^T|$ have grouping effect. 
\begin{proof}
The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
z_{pi}^*-z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (W_{pi}-W_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
|Z_{pi}^*-Z_{pj}^*| & \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 + \alpha_2 |(W_{pi}-W_{pj})|}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2 + \alpha_2 |W_{pi}-W_{pj}|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $|W_{pi}-W_{pj}| \rightarrow 0$.
Then $|Z_{pi}^*-Z_{pj}^*| \rightarrow 0$ and
$(Z^*)^T$ has grouping effect.
Since $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \leq |Z_{pi}^*-Z_{pj}^*|$, $|(Z^*)^T|$ also has grouping effect.
\end{proof}
\end{lemma}

\begin{lemma}
\label{lemma4}
Matrix $\tilde{Z}$ has grouping effect. 
\begin{proof}
From Lemma~\ref{lemma:z-star-abs} and~\ref{lemma3},
both $\lvert Z^*\rvert$ and $\lvert (Z^*)^T\rvert$ have the grouping effect.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
\begin{equation}
\begin{split}
\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert & = \frac{\bigl| (|Z^*_{ip}|+|Z^*_{pi}|) - (|Z^*_{jp}|+|Z^*_{pj}|)\bigr|}{2} \\
& \leq \frac{\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| + \bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr|}{2}
\end{split}
\end{equation}
If $x_i \rightarrow x_j$,
both $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \rightarrow 0$,
so $\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert \rightarrow 0$ and
$\tilde{Z}$ has grouping effect.
\end{proof}
\end{lemma}


\comment{
\begin{lemma}
\label{lemma3}
$(Z^*)^T$ has the grouping effect. 

Proof. The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
z_{pi}^*-z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (W_{pi}-W_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
||Z_{pi}^*-Z_{pj}^*||_2 & \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 + \alpha_2 ||(W_{pi}-W_{pj})||_2}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2 + \alpha_2 ||W_{pi}-W_{pj}||_2}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $||W_{pi}-W_{pj}||_2 \rightarrow 0$.
Then $||Z_{pi}^*-Z_{pj}^*||_2 \rightarrow 0$,
which proves the grouping effect of $(Z^*)^T$.
%\begin{equation}
%\begin{split}
%||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 & \leq ||\bmx_p^TY(X^T(\bmx_i-\bmx_j) +\alpha_2(\bm{w}_i - \bm{w}_j))||_2\\
%& \leq ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2 +\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2\\
%\end{split}
%\end{equation}
\end{lemma}

\begin{lemma}
\label{lemma4}
$\tilde{Z}$ has the grouping effect. 

Proof. From Lemma~\ref{lemma2} and~\ref{lemma3},
both $Z^*$ and $(Z^*)^T$ have the grouping effect,
which can be easily extended to
$|Z^*|$ and $|(Z^*)^T|$.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
$\tilde{Z}$ also has the grouping effect.
\end{lemma}

To this end, we summarize ROSC as follows.
ROSC first computes the TKNN graph $\mathcal{G}$
and the associated weight matrix $\mathcal{W}_K$. Then it applies power iteration to generate $p$
pseudo-eigenvectors that form a $p \times n$ matrix $X$.
After whitening and normalization on $X$,
the coefficient matrix $Z^*$ can be calculated by solving Eq.~\ref{eq:solution},
which further leads to the construction of a rectified similarity matrix $\tilde{Z}$.
Since $\tilde{Z}$ has the grouping effect, 
the standard spectral clustering methods (e.g., NCuts) will be finally applied to derive more robust clustering results.
The time complexity of ROSC will be no more than the standard spectral clustering methods,
which is $O(n^3)$ in general.
In the future, we will attempt to improve it. 
}

\begin{algorithm}
\begin{small}
\caption{ROSC}
\label{alg}
\begin{algorithmic}[1]
\Require $S$, $k$.
\Ensure $\mathcal{C} = \{C_1, ..., C_k\}$
\State Compute TKNN graph $\mathcal{G}$ and reachability matrix $\mathcal{W}$
\State Normalize the similarity matrix $S$ by $W = D^{-1}S$
%\For $j \leftarrow 1$ do
%\State$t = 0$
%\Repeat
%\State $v_j^{t+1} \leftarrow \frac{Wv_j^t}{||Wv_j^t||_1}$
%\State $ \delta^{t+1} \leftarrow |v_j^{t+1} - v_j^t|$
%\State $t$++
%\Until $||\delta_j^t+1 - \delta_j^t||_{max} \leq \epsilon$ or $t\geq T$
%\EndFor
\State Apply PI on $W$ and generate $p$ pseudo-eigenvectors $\{\bm{v}_r\}_{r=1}^p$
\State $X = \{\bm{v}_1^T; \bm{v}_2^T; ...; \bm{v}_p^T\}$; $X$ = whiten($X$)
\State Normalize each object feature vector
\State Solve Eq.~\ref{eq:solution} to obtain the coefficient matrix $Z^*$
\State Construct a rectified similarity matrix $\tilde{Z} = (|Z^*| + |Z^*|^T)/2$
\State Run standard spectral clustering methods, e.g., NCuts, with $\tilde{Z}$ as the
similarity matrix to obtain a clustering $\mathcal{C} = \{C_r\}_{r=1}^k$
%\State Decode $\{C_r\}_{r=1}^k$ from $\{{\bm z_r}\}_{r=1}^k$
\State \Return $\mathcal{C} = \{C_1, ..., C_k\}$
\end{algorithmic}
\end{small}
\end{algorithm}









==> tex/algorithm_report1.tex <==
\section{Algorithm}
\label{sec:algorithm}

In this section we describe our ROSC algorithm. Figure~\ref{figure:flow_graph}(c) shows a 
flow diagram of ROSC. ROSC follows the basic pipeline of spectral clustering except that
it generates a coefficient matrix $Z$ 
%(shown in the red box of the diagram) 
and feeds it
 into the clustering pipeline in place of
the similarity matrix $S$. 
The objective is to find a  $Z$ that possesses  grouping effect. 
To achieve that, ROSC uses PI to obtain {\pev}s from which a basic $Z$ is derived.
Next, it generates the TKNN graph with which $Z$ is rectified. 
In the following, we discuss how $Z$ is derived from the {\pev}s, define the TKNN graph,
describe the rectification process, 
and prove that the resulting $Z$ has the desired grouping effect. 

%
%In this section, we propose a \textbf{RO}bust \textbf{S}pectral \textbf{C}lustering method ROSC. 
%Instead of directly performing spectral clustering on the given similarity matrix, 
%it constructs a new matrix that reserves the efficacy of effective similarities 
%and rectifies ineffective ones in the raw similarity matrix.
%The new matrix will lead to a more robust spectral clustering.

\comment{
\subsection{Model overview}
The overall framework of ROSC is summarized as follows.

First, generate a set of pseudo-eigenvectors.
Since the standard spectral clustering methods using only the dominant eigenvectors may fail 
in the data containing multi-scale clusters,
we generate a set of pseudo-eigenvectors to fuse more useful cluster-separation information.

Second, rectify the given similarity matrix.
The failure of spectral clustering on multi-scale data originates from the inaccurate similarity matrix.
Therefore, we rectify the matrix and aim to achieve a new one
that can more accurately reflect the true similarities between objects.
%This is a major problem to be addressed.

Third, perform spectral clustering.
After rectification, the new similarity matrix will be more accurate and it will be safer to perform spectral clustering. 

These three steps will lead to robust clustering results and next we introduce each step in detail.
}

\subsection*{Pseudo-Eigenvectors}
\label{sec:sec:pseudo}
Given a similarity matrix $S$, we normalize it by $D^{-1}S$ and apply PI to obtain {\pev}s.
%When dealing with multi-scale data,
%spectral clustering
%using only the top-$k$ eigenvectors may fail while some other eigenvectors may be useful~\cite{lin2010power}.
%Therefore, it is necessary to fuse the discriminative cluster-separation information in all eigenvectors
%and PI provides such fusion by returning a pseudo-eigenvector.
%However, when the number of clusters is large,
%a single pseudo-eigenvector is insufficient due to the cluster-collision problem. 
%%Since PI returns a pseudo-eigenvector that is a combination of all the eigenvectors,
Similar to~\cite{ye2016fuse},
we run PI multiple times with different random initial vectors to generate a set of {\pev}s, 
which maps each object into a low dimensional embedding.
Note that small {\ev}s are {\it shrunk} by PI~\cite{lin2010power}.
%\footnote{From Equation~\ref{eq:pi}, we see that the $i$-th 
%largest \ev\ is 
%shrunk at a rate of $\lambda_i/\lambda_1$ per iteration.}.
To alleviate the shrinkage of small {\ev}s,
we follow the approach of~\cite{huang2014diverse}
and gradually decrease the number of iterations executed in PI as more {\pev}s are obtained. 

Since the {\pev}s approximate the most dominant {\ev}, they could be similar. 
To reduce this redundancy,
whitening~\cite{kessy2017optimal} is used to make the pseudo-eigenvectors uncorrelated.
Moreover, noise in the {\pev}s are reduced 
by a rectification process, which will be discussed later.

\comment{
First, we generate a set of pseudo-eigenvectors using different random vectors $\bm{v}_0$.
From Eq.~\ref{eq:v0}, $\bm{v}_0$ can be represented by the subspace spanned by all the eigenvectors.
Suppose $\bm{e}_i$ is an informative eigenvector with a relatively small eigenvalue $\lambda_i$.
Given a $\bm{v}_0$, if it has a dominant component in the direction of $\bm{e}_i$, 
i.e., the associated coefficient $c_i$ is large, 
with an appropriate number of iterations, $c_i\lambda_i^t\approx c_2\lambda_2^t$,
the effect of $\bm{e}_i$ will be finally retained in the pseudo-eigenvector.
Therefore, multiple pseudo-eigenvectors generated by different $\bm{v}_0$
may increase the chance to hold all the informative eigenvectors.

Second, we can control the number of iterations in PI.
In PIC, the \emph{velocity} and \emph{acceleration} at the $t$-th iteration are respectively defined as
$\bm{\delta}_t = \bm{v}_t - \bm{v}_{t-1}$ and $\bm{\epsilon}_t = \bm{\delta}_t-\bm{\delta}_{t-1}$.
A threshold $\epsilon$ is introduced to measure the acceleration change in two consecutive iterations 
and stop PI when $|\bm{\epsilon}_t-\bm{\epsilon}_{t-1}|<\epsilon$.
However,
since the effect of eigenvectors corresponding to smaller eigenvalues will shrink as $t$ increases,
we can decrease the number of iterations by gradually increasing the $\epsilon$ value,
which provides another way to keep useful information in ``less important'' eigenvectors. 
}

\subsection*{Transitive {\it K} Nearest Neighbor (TKNN) Graph}

%\begin{figure}
%    \centering
%        \includegraphics[width = 0.8\linewidth]{figure/example1.eps}
%        \caption{An toy example}
%        \label{figure:example1}
%\end{figure}

%The \emph{$K$ nearest neighbor} (KNN) graph is generally used to depict the most adjacent relations between objects,
%in which the linked objects are generally assumed to share common characteristics.
%Given a set of objects $\mathcal{X} = \{\bm{x}_1,\bm{x}_2,...,\bm{x}_n\}$,
%the KNN graph $G_{K} = (V, E)$ is a graph with $V = \mathcal{X}$ and $E = \{e_{ij}\}$.
%%An edge $e_{ij}$ between $\bm{x}_i$ and $\bm{x}_j$ indicates
%%$x_j \in N_K(\bm{x}_i)$ or $x_i \in N_K(\bm{x}_j)$,
%%where $N_K(\bm{x}_i)$ denotes the set of $K$ nearest neighbors of $\bm{x}_i$.
%%at least one of the two end nodes is in the $K$ nearest neighborhood of the other.
%%However, the $K$ nearest neighborhood relation is not symmetric,
%%i.e., $x_j \in N_K(\bm{x}_i)$ is inequivalent to $x_i \in N_K(\bm{x}_j)$, 
%Some previous work~\cite{yin2016laplacian} simply considers $e_{ij}$
%exists when $\bmx_j \in N_K(\bmx_i)$ or $x_i \in N_K(\bmx_j)$,
%where $N_K(\bmx_i)$ denotes the set of $K$ nearest neighbors of $\bmx_i$.
%However,
%in the case of data containing multi-scale clusters,
%such definition may lead to an edge between
%two objects in different clusters.
%Fig.~\ref{figure:example1} shows an toy example which consists of two multi-scale clusters
%marked by ``$\times$" and ``$+$" respectively.
%For object $\bmx_1$,
%object $\bmx_2$ is its nearest neighbor.
%But for $\bmx_2$, $\bmx_1$ is far away from it.
%In this case, there will be an edge between $\bmx_1$ and $\bmx_2$ in the traditional KNN graph.
%However, since $\bmx_1$ and $\bmx_2$ belong to different clusters,
%they should not be connected.

Our objective is to capture the high correlations between objects that belong to the same cluster even 
 though the objects could be located at distant far ends of a cluster. 
 These correlations are expressed via a TKNN graph, which is used to 
 regularize the coefficient matrix $Z$.

\begin{definition}
\label{def:nei_relation}
\textbf{(Mutual  $K$-nearest neighbors)}
Let $N_K(x)$ be the set of $K$ nearest neighbors of an object $x$.
Two objects $x_i$ and $x_j$ are said to be mutual $K$-nearest neighbors of each other,
denoted by $x_i \sim x_j$, 
iff $x_i \in N_K(x_j)$ and $x_j \in N_K(x_i)$.
\hfill$\Box$
\end{definition}

%In the case of multi-scale data,
%the KNN graph is sometimes insufficient to reflect whether two objects belong to the same cluster or not.
%For example, objects $\bmx_2$ and $\bmx_3$ in Fig.~\ref{figure:example1} belong to the same cluster, 
%but they are both far away from each other.
%%objects $x_1$ and $x_2$ are in different clusters despite their closeness.
%To construct an effective KNN graph, $\bmx_2$ and $\bmx_3$
%are expected to be linked.
%Therefore,
%the reachability between two objects is introduced.

\begin{definition}
\label{def:reachability}
\textbf{(Reachability)}
Two objects $x_i$ and $x_j$ are said to be reachable from each other
if there exists a sequence of $h \geq 2$ objects 
 $\{x_i = x_{a_1}, \ldots, x_{a_h} = x_j\}$ such that
 $x_{a_r} \sim x_{a_{r+1}}$ for $1 \leq r < h$.
 \hfill$\Box$
\end{definition}

\begin{definition}
\label{def:trans_relation}
\textbf{(Transitive $K$-nearest neighbor (TKNN) graph)}
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
the TKNN graph $\mathcal{G}_K = (\mathcal{X},\mathcal{E})$
is an undirected graph
where $\mathcal{X}$ is the set of vertices and $\mathcal{E}$ is the set of edges.
Specifically, the edge ($x_i$, $x_j$) $\in \mathcal{E}$
iff $x_i$ and $x_j$ are reachable from each other.
We represent the TKNN graph by an $n \times n$ {\it reachability matrix}
$\mathcal{W}$ 
whose ($i$,$j$)-entry $\mathcal{W}_{ij} = 1$ if ($x_i$, $x_j$) $\in \mathcal{E}$; 0 otherwise.
\hfill$\Box$
\end{definition}

%We note that mutual-KNN is a symmetric relation and so is reachability. 

%Compared with the traditional KNN graph, 
%the TKNN graph can more accurately reflect 
%whether two objects belong to the same cluster or not.
%It will be used in the next section to rectify the matrix of similarity between objects.
 
\subsection*{Coefficient Matrix}
%In the case of multi-scale data,
%the distance-based similarity is likely to be ineffective. 
%To improve the clustering performance,
%it is necessary to rectify the matrix.
%The rectification should follow two principles.
%First, for the effective similarities, the efficacy should be reserved.
%Second, for the ineffective ones, the efficacy should be enhanced.
%For example,
%the closeness between objects $\bmx_3$ and $\bmx_4$ in Fig.~\ref{figure:example1}
%leads to a large similarity value.
%Since the two objects are of the same cluster,
%the new value should still be large.
%In comparison, 
%both the similarity between $\bmx_1$ and $\bmx_2$ and the one between $\bmx_2$ and $\bmx_3$
%should be rectified, as these distance-based similarities are ineffective.

%In the multi-scale data,
%different clusters may have different sizes, densities or even geometric structures.
The similarity between two objects describes the degree to which they share common characteristics.
The more similar they are, 
the more likely that one object can be represented by the other. 
Therefore,
to depict the relationships between objects in multi-scale data,
each object is linearly characterized by other objects,
assuming the well-known linear subspace model~\cite{liu2013robust}.

We generate $p$ {\pev}s using PI. 
%just as a non-linear manifold can be locally approximated by linear subspaces.
%First, these vectors, which retain the effects of dominant eigenvectors,
%can certainly retain the original accurate similarities between objects.
%Second, they absorb the cluster-separation information from the seemingly ``less important'' eigenvectors,
%which further provides a reliable source of information to rectify the erroneous similarities.
Let $X\in \mathcal{R}^{p\times n}$ be a matrix whose rows are the {\pev}s.
The $q$-th column of $X$ can be taken as a feature vector $\bmx_q$ of an object $x_q$.
We normalize the column vectors of $X$ such that $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$.
We determine a coefficient matrix $Z \in \mathcal{R}^{n \times n}$ by\footnote{We will regularize $Z$ to avoid the trivial solution of $Z$ being the identity matrix.}
\begin{equation}
\label{eq:nonoise}
X = XZ.
\end{equation} 
One can interpret $Z_{ij}$ 
as a value that reflects how well object $x_i$ characterizes object $x_j$.
%To avoid the trivial solution of $Z$ equalling the identity matrix,
%we will regularize $Z$ later.
%For simplicity, we do not explicitly mention this constraint in the rest of the paper.

As indicated by previous works~\cite{ye2016fuse}, the generated pseudo-eigenvectors are likely to be noise-corrupted.
We thus extend Equation~\ref{eq:nonoise} by introducing a noise matrix $O$, giving:
%However, although the pseudo-eigenvectors inherit useful cluster-separation information,
%they may also be contaminated by noise.
%Thus a matrix $O$ is introduced to capture the noise,
\begin{equation}
X = XZ + O.
\label{eq:O}
\end{equation} 
%The TKNN graph conveys information on whether two objects belong to the same cluster or not,

As we have explained, the TKNN graph  conveys useful clustering information, bringing highly
correlated objects that are located at distant far ends of a cluster together.
We thus use the TKNN graph to regularize matrix $Z$.
We derive the following objective function:
%Since our objective is to derive a $Z$ which can better reflect the true similarities between objects,
\comment{
\begin{equation}
%\label{eq:obj}
\min_Z ||O||_F^2+\lambda_1||Z||_F^2 + \lambda_2||Z-\mathcal{W}_K||_F^2,
s.t., X = XZ+O,
\end{equation}
}
%By substituting $O$, we derive
\begin{equation}
\label{eq:obj_constraint}
\min_Z ||X-XZ||_F^2 + \alpha_1 ||Z||_F^2 + \alpha_2 ||Z-\mathcal{W}||_F^2,
\end{equation}
where $\alpha_1 > 0,\alpha_2 \geq 0$ are two 
weighting factors that adjust the relative weights of the three components that constitute
the objective function.
The objective function consists of three terms.
The first term aims to reduce the noise matrix $O$ (see Equation~\ref{eq:O}),
the second term is the Frobenius norm on $Z$, and
%that restricts any item in $Z$ from being dominant.
the third term regularizes $Z$ by the TKNN graph.
%For simplicity, as in~\cite{lu2012robust},
%we remove the constraint and formulate the problem as
%\begin{equation}
%\label{eq:obj}
%\min_Z ||X-XZ||_F^2 + \lambda_1 ||Z||_F^2 + \lambda_2 ||Z-\mathcal{W}_K||_F^2.
%\end{equation}
%$\lambda_1$ and $\lambda_2$ are two parameters to balance the effects of three parts.
A closed-form solution, $Z^*$, to the optimization problem is
\begin{equation}
\label{eq:solution}
Z^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^TX+\alpha_2\mathcal{W}).
\end{equation}

\subsection*{Grouping Effect}
For an object $x_p$, 
let $\bmz_p$ be the $p$-th column of the coefficient matrix $Z$.
We interpret the entries of $\bmz_p$ as the coefficients that express $x_p$ as a linear combinations
of other objects. 
Previous works~\cite{lu2012robust,lu2013correlation,hu2014smooth} have shown that if $Z$ has {\it grouping effect}, then performing spectral 
clustering based on $Z$ would be effective. 
Intuitively, $Z$ has grouping effect if, given two {\it highly correlated} objects $x_i$ and $x_j$,
their characterizations of other objects are similar.
Existing works mostly consider {\it high correlation} between objects as {\it high similarity} of their
feature vectors. With ROSC, we consider object similarity in terms of both feature similarity and 
reachability similarity. 
Feature similarity is measured by the objects' feature vectors as given by the columns of matrix $X$.
Reachability similarity is measured by the columns of matrix $\mathcal{W}$, 
each of which shows the reachability of an object to all others. 
Formally,



%It has been shown that the first two terms in the objective function decide the \emph{grouping effect} of $Z$~\cite{lu2012robust}.
%In Problem~\ref{eq:obj}, the first two terms decides whether $Z$ has the grouping effect~\cite{lu2012robust} defined as follows.
%i.e., the more highly correlated two objects are,
%the larger weight one will have in characterizing the other~\cite{lu2012robust}.

\begin{definition}
\label{def:grouping}
\textbf{(Grouping effect)}. 
Given a set of objects $\mathcal{X} = \{x_1, x_2,..., x_n\}$,
let $\bmw_q$ be the $q$-th column of $\mathcal{W}$. 
Further, let $\xarrow{i}{j}$ denote the condition:
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and 
(2) $\lVert \bmw_i - \bmw_j \rVert_2 \rightarrow 0$.
A matrix $Z$ is said to have grouping effect
if
\[
\xarrow{i}{j} \Rightarrow |Z_{ip} - Z_{jp}| \rightarrow 0\; \forall 1 \leq p \leq n.
\]
%for an arbitrary object $\bmx$ and its associated coefficient vector $\bm{z}$,
%If $\bmx_i\rightarrow \bmx_j$,
%then $z_{pi}\rightarrow z_{pj}$,
%where $z_{pi}$ and $z_{pj}$ are the $i$th and $j$th entry in $\bm{z}_p$ respectively.
%Then we say the self-representation matrix $Z$
%has the grouping effect.
%\hfill$\Box$
\end{definition}

Our next task is to prove that the optimal solution $Z^*$ (as given in Equation~\ref{eq:solution})
% of Equation~\ref{eq:obj_constraint}
has the grouping effect.
In the following discussion, we use $\bmz_q^*$ to denote the $q$-th column vector of $Z^*$.

\begin{lemma}
\label{lemma1}
Given a set of objects $\mathcal{X}$,
the matrix
$X\in \mathcal{R}^{p\times n}$ that is composed of the {\pev}s as rows,
 the reachability matrix $\mathcal{W}$,
 and the optimal soution $Z^*$ of Equation~\ref{eq:obj_constraint},
\begin{equation}
\label{eq:zi}
Z_{ip}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 \mathcal{W}_{ip}}{\alpha_1+\alpha_2}, \;\;\; \forall 1 \leq i, p \leq n.
\end{equation}
\end{lemma}

\begin{proof}
For $1 \leq p \leq n$,
let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \alpha_1 ||\bm{z}_p||_2^2 + \alpha_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
Since $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have $\frac{\partial{J}}{\partial{Z}_{ip}}|_{\bm{z}_p = \bm{z}_p^*} = 0\; \forall 1\leq i \leq n$.
Hence, $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\alpha_1Z_{ip}^*+2\alpha_2(Z_{ip}^*-\mathcal{W}_{ip}) = 0$,
which induces Equation~\ref{eq:zi}.
\end{proof}

%\begin{lemma}
%\label{lemma1}
%Given a set of objects $X\in \mathcal{R}^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object and $\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bmx_p$.
%Each item $z_{pi}^*$ in the optimal solution $\bm{z}_p^*$ to the problem 
%$\min_{\bm{z}} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$ is
%\begin{equation}
%\label{eq:zi}
%z_{pi}^* = \frac{\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*) + \lambda_2 w_{pi}}{\lambda_1+\lambda_2},
%\end{equation}
%where $w_{pi} = 1$, if $\bm{x_p}$ and $\bm{x}_i$ are reachable; $0$, otherwise. 
%
%Proof. Let $J(\bm{z}_p) =  ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Since $\bm{z}_p^*$ is the optimal solution, then $\frac{\partial{J}}{\partial{z}_{pi}}|_{\bm{z}_p = \bm{z}_p^*} = 0$.
%Thus we have $-2\bm{x}_i^T(\bm{x}_p-X\bm{z}_p^*)+2\lambda_1z_{pi}^*+2\lambda_2(z_{pi}^*-w_{pi}) = 0$,
%which induces Eq.~\ref{eq:zi}.
%\end{lemma}

\comment{
Eq.~\ref{eq:zi} calculates the weight of object $\bm{x}_i$ in characterizing $\bm{x}$.
For $w_i$, if $\bm{x}$ and $\bm{x}_i$ are reachable in the TKNN graph, $w_i = 1$; otherwise, $w_i = 0$. 
Eq.~\ref{eq:zi} rectifies the ineffective similarity as follows.
When $\bm{x}$ and $\bm{x_i}$ are far away from each other in the feature space
but reachable in the TKNN graph,
$z_i$ will be increased by $w_i = 1$.
%which rectifies the original incorrect similarity value between them.
Moreover, if $\bm{x}$ and $\bm{x}_i$ are highly correlated,
the first two terms in the problem can decide a large $z_i$,
even in the case that they are unreachable.
%$z_i$ can still keep large with a small $\lambda_2$.
In summary, Eq.~\ref{eq:zi} can not only hold the original accurate similarities but also rectify the incorrect ones.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space but connected in the TKNN graph, 
their similarity will be increased.

\noindent{\small$\bullet$}
For any two objects dissimilar in the feature space and disconnected in the TKNN graph, 
their similarity will be further decreased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space and connected in the TKNN graph,
their similarity will be further increased.

\noindent{\small$\bullet$}
For any two objects similar in the feature space but disconnected in the TKNN graph,
their similarity will be decreased. In this case,
provided that the raw similarity is effective already,
even though the new value will be decreased,
but it will be still
}

\begin{lemma}
\label{lemma2}
%Given a set of objects $X\in R^{d\times n}$ and a TKNN graph $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathcal{W}_K)$,
%let $\bm{x}_p$ be an arbitrary object, 
%$\bm{w}_p$ be the column vector in $\mathcal{W}_K$ describing the connectivity of $\bm{x}_p$, and
%$\bm{z}_p^*$ be the optimal solution to the problem 
%$\min_{\bm{z}_p} ||\bm{x}_p-X\bm{z}_p||_2^2 + \lambda_1 ||\bm{z}_p||_2^2 + \lambda_2 ||\bm{z}_p-\bm{w}_p||_2^2$.
%Assume all the objects have been normalized.
%For any two objects $\bm{x}_i$ and $\bm{x}_j$,
$\forall 1 \leq i, j, p \leq n$,
\begin{equation}
\label{eq:norm}
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)} + \alpha_2|\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2},
\end{equation}
where $c = \sqrt{1+\alpha_2||\bm{w}_p||_2^2}$ and $r = \bm{x}_i^T\bm{x}_j$.
\end{lemma}

\begin{proof}
From Equation~\ref{eq:zi}, we have 
\begin{equation}
\nonumber
Z_{ip}^*-Z_{jp}^* = \frac{(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*) + \alpha_2 (\mathcal{W}_{ip}-\mathcal{W}_{jp})}{\alpha_1+\alpha_2}.
\end{equation}
That implies 
\begin{small}
\begin{equation}
\label{eq:zizj}
\begin{split}
|Z_{ip}^*-Z_{jp}^*| & \leq \frac{|(\bm{x}_i^T - \bm{x}_j^T)(\bm{x}_p-X\bm{z}_p^*)| + \alpha_2 |\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bm{x}_i - \bm{x}_j||_2||\bm{x}_p-X\bm{z}_p^*||_2 + \alpha_2 |\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
\end{small}

Since the column vectors of $X$ are normalized (i.e., $\bmx_q^T \bmx_q = 1 \; \forall 1 \leq q \leq n$) , we have
$||\bm{x}_i - \bm{x}_j||_2 = \sqrt{2(1-r)}$,
where $r = \bm{x}_i^T\bm{x}_j$.
%measuring the closeness between $\bm{x}_i$ and $\bm{x}_j$ in the feature space.
%As $\bm{z}_p^*$ is the optimal solution, 
As $Z^*$ is the optimal solution of Equation~\ref{eq:obj_constraint}, we have
\begin{equation}
\begin{split}
J(\bm{z}_p^*) & = ||\bm{x}_p-X\bm{z}_p^*||_2^2 + \alpha_1 ||\bm{z}_p^*||_2^2 + \alpha_2 ||\bm{z}_p^*-\bm{w}_p||_2^2 \leq  \\
J(\bm{0}) & = ||\bm{x}_p||_2^2 + \alpha_2 ||\bm{w}_p||_2^2 = 1 + \alpha_2 ||\bm{w}_p||_2^2.
\end{split}
\end{equation}
Hence, $||\bm{x}_p-X\bm{z}_p^*||_2 \leq \sqrt{1 + \alpha_2 ||\bm{w}_p||_2^2} = c$.
Equation~\ref{eq:zizj} can be further simplified as
\begin{equation}
\nonumber
|Z_{ip}^*-Z_{jp}^*| \leq \frac{c\sqrt{2(1-r)}+ \alpha_2 |\mathcal{W}_{ip}-\mathcal{W}_{jp}|}{\alpha_1+\alpha_2}.
\end{equation}
\end{proof}

\begin{lemma}
Matrix $Z^*$ has grouping effect.
\label{lemma:z-star}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$ such that $\xarrow{i}{j}$,
we have,  %by definition, 
(1) $\bmx_i^T \bmx_j \rightarrow 1$ and (2) $||\bmw_{i}-\bmw_{j}||_2 \rightarrow 0$.
These imply
$r = \bmx_i^T \bmx_j \rightarrow 1$ and  $|\mathcal{W}_{ip}-\mathcal{W}_{jp}| \rightarrow 0$.
Hence, the two terms of the numerator of the R.H.S of Equation~\ref{eq:norm} are close to 0. 
Therefore, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$ and thus $Z^*$ has grouping effect.
\end{proof}

Indeed, Equation~\ref{eq:norm} shows how our algorithm ROSC enhances the effectiveness of 
spectral clustering on multi-scale data. 
Comparing with traditional approaches, which focus on feature similarity, ROSC uses $Z^*$
to integrate feature similarity  ($r$) with
reachability similarity ($|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$).
In particular, two distant objects $x_i$ and $x_j$ of a cluster may not share a strong feature similarity.
This leads to a small $r$ and traditional approaches will likely put them into separate clusters.
On the contrary, ROSC considers the strong reachability of the objects
to derive a small value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$, and thus keeping them in the same cluster.
Moreover, for $x_i$ and $x_j$ that belong to two different dense clusters but happen to be close in 
space (i.e., $x_i$ and $x_j$ have strong feature similarity), 
traditional approaches may inadvertently merge them into the same cluster. 
ROSC, however, would discover their low reachability (via the mutual-KNN relation)
and derive a large value of $|\mathcal{W}_{ip}-\mathcal{W}_{jp}|$.
This regulates matrix $Z^*$ and avoids the incorrect merging.
As we will see in the next section, ROSC's approach 
greatly improves clustering quality and is more robust than other algorithms in handling
multi-scale data.
 
%Lemma~\ref{lemma1} and~\ref{lemma2} prove the grouping effect of $Z^*$ derived by Eq.~\ref{eq:solution}.
%%the weight difference of two objects in characterizing an arbitrary object $\bm{x}$ is bounded.
%Given two objects $\bmx_i$ and $\bmx_j$, if $\bmx_i \rightarrow \bmx_j$, 
%i.e., $\bmx_i^T \bmx_j \rightarrow 1$ and $||w_{pi}-w_{pj}||_2 \rightarrow 0$,
%then $||z_{pi}^*-z_{pj}^*||_2 \rightarrow 0$.
%%which shows the grouping effect of $Z$ derived by Eq.~\ref{eq:solution}.
%%However, in the case of (1) $\bm{x}_i^T\bm{x}_j = 0$ but $w_i=w_j=1$ and 
%%(2) $\bm{x}_i^T\bm{x}_j = 1$ but $||w_i-w_j||_2=1$,
%%$||z_i^*-z_j^*||_2$ can still be small with an appropriate setting on $\lambda_1$ and $\lambda_2$.
%%Further, since $Z$ can not only retain the accurate similarities but also rectify the incorrect ones, 
%%In other words, objects in the same cluster will be better reflected in the rectified matrix.
%%Such grouping effect together with The rectification ability could guarantee a more robust clustering performance.
%We then summarize how the TKNN graph rectifies the raw similarity matrix.
%Given any two objects $\bmx_i$ and $\bmx_j$,
%\begin{enumerate}[label=(\arabic*), leftmargin=*]
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\setlength{\parskip}{0pt}
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be increased.
%\item $\bmx_i^T \bmx_j \rightarrow 0$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be further decreased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are reachable, the effect of $S_{ij}$ will be further increased.
%\item $\bmx_i^T \bmx_j \rightarrow 1$, $\bmx_i$ and $\bmx_j$ are unreachable, the effect of $S_{ij}$ will be decreased.
%\end{enumerate}
%Among the four cases,
%$Z$ reserves the efficacy of effective similarities by (2) and (3)
%while it enhances the efficacy of ineffective similarities by (1) and (4). 
%Thus spectral clustering based on $Z$ will be more robust.

\comment{
\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 0$ but reachable, $S_{ij}$ will be increased.

\noindent{\small$\bullet$}
%For any two objects dissimilar in the feature space and disconnected in the TKNN graph, their similarity will be further decreased.
$\bmx_i^T \bmx_j \rightarrow 0$ and unreachable, $S_{ij}$ will be further decreased.

\noindent{\small$\bullet$}
%For any two objects similar in the feature space and connected in the TKNN graph, their similarity will be further increased.
$\bmx_i^T \bmx_j \rightarrow 1$ and reachable, $S_{ij}$ will be further increased.

\noindent{\small$\bullet$}
$\bmx_i^T \bmx_j \rightarrow 1$ but unreachable, $S_{ij}$ will be decreased.
}

\subsection*{ROSC: Robust Spectral Clustering}
%The coefficient matrix $Z$ take advantage of both cluster-separation information in all the eigenvectors
%and the TkNN graph, which not only retains the original accurate similarities but also rectifies the incorrect ones.

We note that the matrix $Z^*$ obtained may be asymmetric and it may contain negative values.
To construct a matrix of object similarity, a common fix~\cite{liu2013robust,lu2012robust} is to 
compute $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$.
After $\tilde{Z}$ is computed, ROSC executes a standard spectral clustering method
(e.g., NCuts) using $\tilde{Z}$ as the similarity matrix in place of $S$.
It can be proved that $|Z^*|$, $|(Z^*)^T|$, and hence $\tilde{Z}$ all have grouping effect.
%Due to space limitations, readers are referred to [XXX] for the proofs. 
Finally, ROSC is summarized in Algorithm~\ref{alg}.

\begin{lemma}
Matrix $|Z^*|$ has grouping effect.
\label{lemma:z-star-abs}
\end{lemma}
\begin{proof}
Given two objects $x_i$ and $x_j$,
we have 
$\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \leq |Z_{ip}^*-Z_{jp}^*|$.
From Lemma~\ref{lemma:z-star},
$Z^*$ has grouping effect, i.e.,
if $x_i \rightarrow x_j$, $|Z_{ip}^*-Z_{jp}^*| \rightarrow 0$.
Thus $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and 
$|Z^*|$ has grouping effect.
\end{proof}

\begin{lemma}
\label{lemma3}
$(Z^*)^T$ and $|(Z^*)^T|$ have grouping effect. 
\begin{proof}
The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
Z_{pi}^*-Z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (\mathcal{W}_{pi}-\mathcal{W}_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
|Z_{pi}^*-Z_{pj}^*| & \leq \frac{|\bmx_p^T(\bm{x}_i - \bm{x}_j)| + |\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)| + \alpha_2 |(\mathcal{W}_{pi}-\mathcal{W}_{pj})|}{\alpha_1+\alpha_2}\\
& \leq \frac{|\bmx_p^T(\bm{x}_i - \bm{x}_j)| + |\bmx_p^TYX^T(\bmx_i-\bmx_j)|}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2|\bmx_p^TY(\bm{w}_i - \bm{w}_j)| + \alpha_2 |\mathcal{W}_{pi}-\mathcal{W}_{pj}|}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p||_2||\bm{x}_i - \bm{x}_j||_2 + ||\bmx_p^TYX^T||_2||\bmx_i-\bmx_j||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY||_2||\bm{w}_i - \bm{w}_j||_2 + \alpha_2 |\mathcal{W}_{pi}-\mathcal{W}_{pj}|}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $|\mathcal{W}_{pi}-\mathcal{W}_{pj}| \rightarrow 0$.
Then $|Z_{pi}^*-Z_{pj}^*| \rightarrow 0$ and
thus $(Z^*)^T$ has grouping effect.
Since $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \leq |Z_{pi}^*-Z_{pj}^*|$, $|(Z^*)^T|$ also has grouping effect.
\end{proof}
\end{lemma}

\begin{lemma}
\label{lemma4}
Matrix $\tilde{Z}$ has grouping effect. 
\begin{proof}
From Lemma~\ref{lemma:z-star-abs} and~\ref{lemma3},
both $\lvert Z^*\rvert$ and $\lvert (Z^*)^T\rvert$ have the grouping effect.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
\begin{equation}
\begin{split}
\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert & = \frac{\bigl| (|Z^*_{ip}|+|Z^*_{pi}|) - (|Z^*_{jp}|+|Z^*_{pj}|)\bigr|}{2} \\
& \leq \frac{\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| + \bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr|}{2}
\end{split}
\end{equation}
If $x_i \rightarrow x_j$,
both $\bigl||Z_{ip}^*|-|Z_{jp}^*|\bigr| \rightarrow 0$ and $\bigl||Z_{pi}^*|-|Z_{pj}^*|\bigr| \rightarrow 0$,
so $\lvert \tilde{Z}_{ip} - \tilde{Z}_{jp}\rvert \rightarrow 0$ and
$\tilde{Z}$ has grouping effect.
\end{proof}
\end{lemma}


\comment{
\begin{lemma}
\label{lemma3}
$(Z^*)^T$ has the grouping effect. 

Proof. The problem is equivalent to if $x_i \rightarrow x_j$, $Z^*_{pi} \rightarrow Z^*_{pj}$.
From Lemma~\ref{lemma1},
\begin{equation}
\nonumber
z_{pi}^*-z_{pj}^* = \frac{\bm{x}_p^T ( \bmx_i - \bmx_j - X(\bm{z}_i^*-\bm{z}_j^*)) + \alpha_2 (W_{pi}-W_{pj})}{\alpha_1+\alpha_2}.
\end{equation}
Since $\bm{z}_i^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_i+\alpha_2\bm{w}_i),\bm{z}_j^* = (X^TX + \alpha_1I + \alpha_2I)^{-1}(X^T\bmx_j+\alpha_2\bm{w}_j)$,
let $Y = X(X^TX + \alpha_1I + \alpha_2I)^{-1}$. Then
\begin{equation}
\begin{split}
||Z_{pi}^*-Z_{pj}^*||_2 & \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 + \alpha_2 ||(W_{pi}-W_{pj})||_2}{\alpha_1+\alpha_2}\\
& \leq \frac{||\bmx_p^T(\bm{x}_i - \bm{x}_j)||_2 + ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2}{\alpha_1+\alpha_2}\\
& + \frac{\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2 + \alpha_2 ||W_{pi}-W_{pj}||_2}{\alpha_1+\alpha_2}\\
\end{split}
\end{equation}
If $x_i \rightarrow x_j$, i.e., $\bmx_i^T\bmx_j \rightarrow 1$ and $||\bm{w}_i - \bm{w}_j||_2 \rightarrow 0$, 
we have
$||\bm{x}_i - \bm{x}_j||_2 \rightarrow 0$ and $||W_{pi}-W_{pj}||_2 \rightarrow 0$.
Then $||Z_{pi}^*-Z_{pj}^*||_2 \rightarrow 0$,
which proves the grouping effect of $(Z^*)^T$.
%\begin{equation}
%\begin{split}
%||\bmx_p^TX(\bm{z}_i^*-\bm{z}_j^*)||_2 & \leq ||\bmx_p^TY(X^T(\bmx_i-\bmx_j) +\alpha_2(\bm{w}_i - \bm{w}_j))||_2\\
%& \leq ||\bmx_p^TYX^T(\bmx_i-\bmx_j)||_2 +\alpha_2||\bmx_p^TY(\bm{w}_i - \bm{w}_j)||_2\\
%\end{split}
%\end{equation}
\end{lemma}

\begin{lemma}
\label{lemma4}
$\tilde{Z}$ has the grouping effect. 

Proof. From Lemma~\ref{lemma2} and~\ref{lemma3},
both $Z^*$ and $(Z^*)^T$ have the grouping effect,
which can be easily extended to
$|Z^*|$ and $|(Z^*)^T|$.
Since $\tilde{Z} = (|Z^*|+|(Z^*)^T|)/2$,
$\tilde{Z}$ also has the grouping effect.
\end{lemma}

To this end, we summarize ROSC as follows.
ROSC first computes the TKNN graph $\mathcal{G}$
and the associated weight matrix $\mathcal{W}_K$. Then it applies power iteration to generate $p$
pseudo-eigenvectors that form a $p \times n$ matrix $X$.
After whitening and normalization on $X$,
the coefficient matrix $Z^*$ can be calculated by solving Eq.~\ref{eq:solution},
which further leads to the construction of a rectified similarity matrix $\tilde{Z}$.
Since $\tilde{Z}$ has the grouping effect, 
the standard spectral clustering methods (e.g., NCuts) will be finally applied to derive more robust clustering results.
The time complexity of ROSC will be no more than the standard spectral clustering methods,
which is $O(n^3)$ in general.
In the future, we will attempt to improve it. 
}

\begin{algorithm}
\begin{small}
\caption{ROSC}
\label{alg}
\begin{algorithmic}[1]
\Require $S$, $k$.
\Ensure $\mathcal{C} = \{C_1, ..., C_k\}$
\State Compute the TKNN graph and the reachability matrix $\mathcal{W}$
\State Calculate $W = D^{-1}S$, where $D_{ii} = \sum_jS_{ij}$
%\For $j \leftarrow 1$ do
%\State$t = 0$
%\Repeat
%\State $v_j^{t+1} \leftarrow \frac{Wv_j^t}{||Wv_j^t||_1}$
%\State $ \delta^{t+1} \leftarrow |v_j^{t+1} - v_j^t|$
%\State $t$++
%\Until $||\delta_j^t+1 - \delta_j^t||_{max} \leq \epsilon$ or $t\geq T$
%\EndFor
\State Apply PI on $W$ and generate $p$ pseudo-eigenvectors $\{\bm{v}_r\}_{r=1}^p$
\State $X = \{\bm{v}_1^T; \bm{v}_2^T; ...; \bm{v}_p^T\}$; $X$ = whiten($X$)
\State Normalize each column vector $\bm{x}$ of $X$ such that $\bm{x}^T\bm{x} = 1$
\State Calculate the coefficient matrix $Z^*$ by Eq.~\ref{eq:solution}
\State Construct $\tilde{Z} = (|Z^*| + |(Z^*)^T|)/2$
\State Run standard spectral clustering methods, e.g., NCuts, with $\tilde{Z}$ as the
similarity matrix to obtain clusters $\mathcal{C} = \{C_r\}_{r=1}^k$
%\State Decode $\{C_r\}_{r=1}^k$ from $\{{\bm z_r}\}_{r=1}^k$
\State \Return $\mathcal{C} = \{C_1, ..., C_k\}$
\end{algorithmic}
\end{small}
\end{algorithm}









==> tex/analysis.tex <==
\section{Analysis}
\label{sec:analysis}
In this section we analyze the structural properties of HINs and classification tasks. We first describe three classification tasks,
which are used in our analysis. Then, we explain the concepts of \chn\ and \cnn, and propose quantitative measures to 
capture these properties.

%In the end of section Introduction, we put forward three questions. Before we involve in the third one to predict whether transductive classification will work on a given HIN or not, we should first investigate the first two which would uncover the factors leading to a good transductive classification. Based on the aforementioned datasets: DBLP, Yago Movie and Freebase Movie, extensive experiments have been conducted, which provides sufficient grounds to our in-depth and logical analysis.

\subsection{Classification tasks}

\textbf{DBLP}\footnote{http://dblp.uni-trier.de/} is a bibliographic information network. 
We extracted a dataset from DBLP that contains 14,376 papers (P), 20 publication venues (V), 14,475 authors (A) and 
8,920 terms (T). 
These form the objects of the HIN. 
There are three types of links, which are authorship (A-P), publication (P-V), and keyword (P-T).
The task is to classify authors into their research areas. 
The label set is \{\emph{database} (DB), \emph{data mining} (DM), \emph{artificial intelligence} (AI) and
\emph{information retrieval} (IR) \}.
%Both \hpm\ and \gm\ use 
We use the set of meta-paths \{APA, APAPA, APVPA, APTPA\} 
as suggested in \cite{DBLP:dblp_conf/kdd/SunNHYYY12}.
%Four research areas: \emph{database}, \emph{data mining}, \emph{artificial intelligence} and \emph{information retrieval} are regarded as labels, and 4057 authors have been labeled by them. Links in the network are of three types: paper-author, paper-venue and paper-term. To classify authors, we use the meta path set $\mathcal{PS}$ = \{APA, APAPA, APVPA, APTPA\} suggested in \cite{DBLP:dblp_conf/kdd/SunNHYYY12} when applying HetPathMine and Grempt.

\textbf{Yago Movie} is a movie related HIN extracted from Yago. The dataset contains 1,465 movies (M), 4,019 actors (A), 1,093 directors (D) and 1,458 writers (W). There are three types of links: M-A, M-D, and M-W. 
All of the extracted movies can be classified into one of three genres: \emph{horror}, \emph{action} and \emph{adventure}.
The task is to label movies into their genres.
We use the meta-path set \{MAM, MDM, MWM, MAMAM, MDMDM, MWMWM\} as suggested
in~\cite{DBLP:dblp_conf/cikm/WanLKYGCH15}.

%All the movies are labeled with regard to three genres: \emph{horror}, \emph{action} and \emph{adventure}. In order to classify movies, similar to \cite{DBLP:dblp_conf/cikm/WanLKYGCH15}, we employ the meta path set $\mathcal{PS}$ = \{MAM, MDM, MWM, MAMAM, MDMDM, MWMWM\}.

\textbf{Freebase Movie} is another movie related HIN extracted from Freebase. 
It consists of 3,492 movies (M), 33,401 actors (A), 2,502 directors (D) and 4,459 producers (P). 
There are three types of links: M-A, M-D, and M-P.
The task is again to label movies into their genres. 
The label set is \{\emph{action}, \emph{adventure} and \emph{crime}\}.
We use the meta-path set \{MAM, MDM, MPM, MAMAM, MDMDM, MPMPM\}~\cite{DBLP:dblp_conf/cikm/WanLKYGCH15}.

\subsection{Structural properties of an HIN}

Transductive classification on networked data utilizes links and paths to evaluate the relatedness of objects.
Objects that are highly related are assumed to share similar labels. 
In a sense, links and paths are used to
propagate labels from labeled objects
to unlabeled ones. 
Algorithms like \gnm\ use the HIN to propagate labels, while algorithms like \hpm\ and \gm\ use
meta-paths to derive TSSNs and propagate labels on those sub-networks. 
In any case, the network structure (of the original HIN or of the derived TSSNs) is
an important factor of the effectiveness of \tcrs.
In particular, 
all these \tcrs\ share the following intrinsic assumption:
\begin{assumption}
{\bf The Connectivity Assumption}.
The structural connectivity between two objects (via links and paths) 
are highly correlated to whether the objects would share the same label. 
\end{assumption}
In this section we address two interesting questions:

{\it Question 1}:
Does the connectivity assumption generally hold for HIN classification tasks?

{\it Question 2}:
If not, how to measure the validity of the connectivity assumption given a classification task?


To answer the first question, we conducted simple experiments on a number of classification tasks.
First, we define {\it true-labeling} using the notations of Definition~\ref{def:labeling}:

\begin{definition}
{\bf True-labeling}.
A labeling $\hat{L}$ is a true-labeling if 
$\forall x \in \mathcal{X}_i$, $\hat{L}(x)$ is the true label (ground truth) of object $x$.
\end{definition}
We put a caret `$\wedge$' on a labeling $L$ to indicate that it is a true-labeling.
For each of the three classification tasks DBLP, Yago Movie and Freebase Movie,
we find the true-labeling $\hat{L}$.
We then cluster objects into the
label-induced clustering $\mathcal{C}_{\hat{L}}$ (see Definition~\ref{def:li-clustering}). 
Each cluster in $\mathcal{C}_{\hat{L}}$ thus contains all and only those objects of a given label.

\begin{table}
\caption{Similarity (NMI) of $\mathcal{C}_{\hat{L}}$ and $\mathcal{C}_{\mathit{NetClus}}$}
\centering
\small
\begin{tabular}{|c|c|c|c|} \hline
 DBLP & Yago Movie & Freebase Movie \\ \hline
$0.707$ & $0.018$ & $0.027$ \\ \hline
\end{tabular}
\label{table:global_nmi}
\end{table}


Next, we apply NetClus~\cite{DBLP:dblp_conf/kdd/SunYH09}, which is a clustering method
that clusters objects in an HIN based on network structure, to our HINs.
For each HIN, we compare the true-label-induced clustering $\mathcal{C}_{\hat{L}}$
(which is based solely on object labels) with
the clustering $\mathcal{C}_{\mathit{NetClus}}$, given by NetClus (which is based solely on network structure).
The similarity of the two clusterings is measured by  
normalized mutual information (NMI).
Table~\ref{table:global_nmi} shows the results.
We see that for DBLP, the NMI is high, indicating that $\mathcal{C}_{\hat{L}}$ and $\mathcal{C}_{\mathit{NetClus}}$
are highly similar. 
In other words, objects that are highly connected (put in the same cluster by NetClus) tend to share the same label
(put in the same cluster by the true-label-induced clustering).
The connectivity assumption is thus strongly valid. 
On the other hand, for Yago Movie and Freebase Movie, the NMI's are very low, indicating that
the connectivity assumption does not hold in those cases.  
This analysis is consistent with the accuracies of the \tcrs\ when they are applied to the three
classification tasks (see Table~\ref{tbl:xlong}).
Our analysis leads to the following conclusion:

\begin{conclusion}
The connectivity assumption does not always hold across HIN classification tasks. When it does, \tcrs\ 
are very effective.
\end{conclusion}

The next question we address is how the validity of the connectivity assumption is evaluated.   
We propose to measure the correlation between {\it structural connectivity of objects} and their {\it label similarity} by 
the concepts of \chn\ and \cnn. 
Intuitively, given a classification task,
an HIN is {\it highly cohesive} if strong connectivity occurs mostly between objects of the same label;
and that the HIN is {\it highly connected} if objects of the same label exhibit strong connectivity.
The correlation between structural connectivity and label similarity is thus high if the HIN is highly cohesive and highly connected.
In the following discussion, we first assume that the true-labeling $\hat{L}$ of a classification task is known.
Cohesiveness and \cnn\ are then defined based on a true-labeling. 
We will discuss in Section~\ref{sec:tester} how the two measures can be estimated when the true-labeling is not known in practice. 

\subsection{Cohesiveness}

Given an HIN $G=(V,E)$,
consider the  task of classifying objects $x \in \mathcal{X}_i$ of type $T_i$ 
with the label set $\mathcal{L} = \{l_1, ..., l_k\}$.
A \tcr\ propagates label from an object $x_u \in \mathcal{X}_i$ to another 
object $x_v \in \mathcal{X}_i$. 
How much this propagation is done depends on the structural connectivity (i.e., links and paths) between $x_u$ and $x_v$.
For example, \hpm\ and \gm\ use meta-paths to derive TSSNs (see Figure~\ref{figure:subnetworks}),
and for each TSSN $G_{\mathcal{P}}$,  which is derived from a meta-path $\mathcal{P}$, 
the structural connectivity between $x_u$ and $x_v$ is measured using \emph{PathSim} \cite{DBLP:dblp_journals/pvldb/SunHYYW11}:

{\small
\begin{equation}
\nonumber
\label{eq:pathsim}
s(x_u, x_v) = \frac{2 \times |\{p_{x_u \leadsto x_v}:p_{x_u \leadsto x_v} \in \mathcal{P}\}|}{|\{p_{x_u \leadsto x_u}:p_{x_u \leadsto x_u} \in \mathcal{P}\}|+|\{p_{x_v \leadsto x_v}:p_{x_v \leadsto x_v} \in \mathcal{P}\}|}.
\end{equation}}

Now, let us consider the true-label-induced clustering $\mathcal{C}_{\hat{L}}$. 
Figure~\ref{figure:special_network} shows an example clustering with 2 clusters (objects with true label `$\Circle$' and those with
true label `$\Box$').
An edge, e.g., ($x_1$,$x_2$), is shown to indicate that two objects are structurally connected
(e.g., they are connected by meta-paths). 
We assume that each edge shown is associated with a weight, which reflects the strength of the connection
(e.g., as measured using \emph{PathSim}).
We call Figure~\ref{figure:special_network} a {\it structural connectivity graph}.

Note that \tcrs\ that use meta-paths 
(such as \hpm\ and \gm) 
measure the connectivity between two
objects based on how well the objects are connected by meta-paths. In this case, the structural connectivity graph can be
seen as a composition (union) of the TSSNs derived from a given set of meta-paths. 
For example, the structural connectivity graph of the movie HIN shown in Figure~\ref{figure:subnetworks}(a)
is the composition of the TSSNs shown in Figures~\ref{figure:subnetworks}(c)-(e).
In particular, the edge connecting M1 and M2 in Figure~\ref{figure:subnetworks}(c) indicates that
M1 and M2 are structurally connected by a meta-path instance (M1-A1-M2).
If M1 is labeled,
the label will be propagated to M2 via the structural connection (M1,M2).
We will discuss how an overall \chn\ value is measured when the structural connectivity graph is a composition of 
multiple TSSNs shortly. For the moment, let us assume that there is only one connectivity graph derived.

As mentioned, 
an HIN is highly cohesive if strong connectivity occurs mostly between objects of the same label.
Referring to Figure~\ref{figure:special_network}, that means 
intra-cluster edges are many-and-strong, while 
inter-cluster edges are few-and-weak.
Figure~\ref{figure:special_network} shows a very cohesive HIN because
there is only one edge ($x_1,y_1$) across the two clusters; most of the structural connections are between objects of the same label.
With this intuition, we quantitatively define \chn\ as follows.


%By exploring the aforementioned questions, we next unveil factors influencing transductive classification in HINs.
%\begin{question}
%In which kinds of heterogeneous information networks will transductive classification perform well?
%\end{question}
%
%Transductive classification on networked data depends on the network structure to propagate labels from labeled objects to unlabeled ones. Moreover, objects with the same label usually have features in common and they can be put in the same cluster. So it is natural to assume that if a network has very good clustering structure, then transductive classification will perform well. A good clustering structure refers to that objects with the same label are densely connected and form a cluster. Furthermore, no inter-cluster edge exists. Such structure will benefit transductive classification in that one labeled object is enough for each cluster to infer labels of all the unlabeled objects within the cluster. Based on the above analysis, we assume:
%
%\begin{assumption}
%When a heterogeneous information network intrinsically has good clustering structure, transductive classification will be effective.
%\end{assumption}
%
%To study the clustering property of the network, labels of objects are taken as the ground truth. We use label to mark the cluster an object belongs to and divide objects to be classified into different clusters. For example, action-genre movies are deemed in the same cluster, authors with research interest on data mining are in the same cluster, etc.
%
%We first validate the assumption by taking the HIN as a whole. Since the network is heterogeneous, traditional clustering methods will not work. We resort to NetClus \cite{DBLP:dblp_conf/kdd/SunYH09}, a specialized clustering method for heterogeneous information network with star schema, to perform clustering. Normalized mutual information (NMI) is used as the measure. The result is shown in table \ref{table:global_nmi}. It is obvious that DBLP network has a better clustering structure than other two datasets, which to some extent reflects our assumption.
%

%To further verify our assumption, we pay attention to meta path. Since meta path has been successfully used in transductive classification methods Grempt and HetPathMine, we can also employ it to measure the clustering property of an HIN. Similarly, given an HIN, we first induce several topology shrinking sub-networks by meta paths. Each sub-network will be homogeneous which contains only the objects of the type to be classified. For each sub-network, objects with the same label are considered in the same cluster. So clusters are same in these sub-networks. As we have mentioned above, if there are more edges within clusters and fewer edges between clusters, then transductive classification will perform well.
%
%After sub-networks have been derived, both HetPathMine and Grempt use \emph{PathSim} \cite{DBLP:dblp_journals/pvldb/SunHYYW11} to measure the similarity between any two objects $x_1$ and $x_2$ in the network. For a meta path $\mathcal{P}$ induced sub-network, \emph{PathSim} is defined as:
%
%{\small
%\begin{equation}
%\nonumber
%\label{eq:pathsim}
%s(x_1, x_2) = \frac{2 \times |\{p_{x_1 \leadsto x_2}:p_{x_1 \leadsto x_2} \in \mathcal{P}\}|}{|\{p_{x_1 \leadsto x_1}:p_{x_1 \leadsto x_1} \in \mathcal{P}\}|+|\{p_{x_2 \leadsto x_2}:p_{x_2 \leadsto x_2} \in \mathcal{P}\}|}
%\end{equation}}
%
%\noindent where $p_{x_1 \leadsto x_2}$ is a path instance between $x_1$ and $x_2$, $p_{x_1\leadsto x_1}$ is that between $x_1$ and $x_1$, and $p_{x_2\leadsto x_2}$ is that between $x_2$ and $x_2$. Then transductive classification is performed on each sub-network and finally integrated. Label propagation heavily depends the weights between objects, the larger the value, the more one will be influenced by the other. Inspired by this, we find that sometimes edge count is not enough to reflect how good transductive classification will be. Larger weights within clusters and smaller weights between clusters are also required. An example is shown in figure \ref{figure:special_network}. There exist a number of intra-cluster edges in both clusters and only one inter-cluster edge between node $A$ and $B$. Suppose the weight on $e_{AB}$ is very large, then weights on other edges in both clusters will be very small. This means that $A$ and $B$ will be greatly influenced by each other. Assume $A$ has been influenced by $B$. After that, even though we know the label of node $C$, it can not propagate to other nodes within the cluster, because it is blocked by $A$.

%\comment{
%\begin{figure}[htbp]
%\centering
%\mbox{
%  \hspace{-0.6cm}
%  \begin{minipage}[t]{0.55\linewidth}
%     %\centering
%     \includegraphics[width = \linewidth]{figure/homo.pdf}
%     \caption{Topology shrinking sub-network}
%     \label{figure:homo}
%  \end{minipage}
%  \begin{minipage}[t]{0.55\linewidth}
%     %\centering
%     \includegraphics[width = \linewidth]{figure/edge_weights.pdf}
%     \caption{A special network}
%     \label{figure:special_network}
%  \end{minipage}
%  }
%\end{figure}
%}
\begin{figure}
    \centering
        \includegraphics[width = 0.5\linewidth]{figure/weights_new.pdf}
        \caption{A structural connectivity graph}
        \label{figure:special_network}
\end{figure}

%Combining intuition and characteristic of transductive classification, we propose that for any two clusters, if intra-cluster edges are dense and inter-cluster edges are sparse, transductive classification will perform well. Here, dense and sparse refer to two measures: the number of edges and the weights of edges. We have mentioned that an HIN can induce several sub-networks and these sub-networks have same clusters indicated by labels. Then we can measure the clustering property in a reverse order of cluster, sub-network and finally HIN.
%\begin{definition}
Given two clusters $C_1$ and $C_2$ in a true-label-induced clustering $\mathcal{C}_{\hat{L}}$,
with respect to a structural connectivity graph,
let $h_1$ ($h_2$) be the number of intra-cluster edges in $C_1$ ($C_2$) with a sum of edge weights
$w_1$ ($w_2$). 
Also, let $h_{1,2}$ be the number of inter-cluster edges between $C_1$ and $C_2$ with a 
sum of edge weights $w_{1,2}$.
Define,
%
%For any two clusters $C_1$ and $C_2$, $C_1$ has $h_1$ intra-cluster edges with total weights $w_1$, $C_2$ has $h_2$ intra-cluster edges with total weights $w_2$. There are $h_{1,2}$ inter-cluster edges between them with total weights $w_{1,2}$. Then
%\emph{intra-inter edge ratio} for each cluster is defined as 
\begin{equation}
\label{eq:edge_ratio}
\rho(C_1) = \frac{h_1}{h_{1,2}+h_1}, \;\;\; \rho(C_2) = \frac{h_2}{h_{1,2}+h_2}, \mbox{  and }
\end{equation}
%\emph{intra-inter edge weights ratio} for each cluster is defined as 
\begin{equation}
\label{eq:weights_ratio}
\eta(C_1) = \frac{w_1}{w_{1,2}+w_1}, \;\;\; \eta(C_2) = \frac{w_2}{w_{1,2}+w_2}. \mbox{        }
\end{equation}
$\rho(C_1)$ can be interpreted as, ``Among all the edges that connect some objects in $C_1$, the fraction of which that connect {\it only}
objects in $C_1$.'' The other quantities can be interpreted similarly. 
%To facilitate label propagation, both ratios are expected to be large enough in both clusters. To avoid that one value is extremely large and others are small, 
We further define the \emph{pairwise cluster cohesiveness} of $C_1$ and $C_2$: 
\begin{equation}
\label{eq:inter-cluster_cohesiveness}
\Upsilon(C_1, C_2) = \rho(C_1) \times \rho(C_2) \times \eta(C_1) \times \eta(C_2).
\end{equation}
%\end{definition}

For a classification task with $k$ labels, 
a labeling induces $k$ clusters $C_1, ..., C_k$.
Let $b_i = |C_i|$.
Define the \emph{cluster cohesiveness} of $C_i$ by
\begin{equation}
\label{eq:cluster_cohesiveness}
\Upsilon_{C_i} = \frac{1}{k-1}\sum_{j\neq i}\Upsilon(C_i, C_j).
\end{equation}
%and the \emph{cohesiveness vector} 
Let $\bm{\Upsilon} = (\Upsilon_{C_1}, ..., \Upsilon_{C_k})^\mathrm{T}$. 
%$\bm{\Upsilon_{G_\mathcal{P}}^\prime} = (\Upsilon_{C_1}, \Upsilon_{C_2}, ..., \Upsilon_{C_N})^\mathrm{T}$. 
We define the \chn\ of an HIN $G$ as the weighted average of the cluster cohesiveness:
%Since $G_\mathcal{P}$ consists of $N$ clusters, then we have \emph{sub-network cluster cohesiveness vector} $\bm{\Upsilon_{G_\mathcal{P}}^\prime} = (\Upsilon_{C_1}, \Upsilon_{C_2}, ..., \Upsilon_{C_N})^\mathrm{T}$. 
%And \emph{sub-network cohesiveness} is the weighted average for clusters:
\begin{equation}
\label{eq:subnetwork_cohesiveness}
\Upsilon_{G} = \bm{\beta}\bm{\Upsilon},
\end{equation}
where $\bm{\beta} = (\frac{b_1}{\sum_{i=1}^k b_i}, \frac{b_2}{\sum_{i=1}^k b_i}, ..., \frac{b_k}{\sum_{i=1}^k b_i})$.

If we use a set of meta-paths $\mathcal{P}_1, ..., \mathcal{P}_r$ in \tc, the structural connectivity graph can be seen as a composition of 
a number of TSSNs $G_{\mathcal{P}_j}$ (1 $\leq j \leq r$).
In this case, we evaluate the cohesiveness of each TSSN to obtain $\Upsilon_{G_{\mathcal{P}_j}}$,
assign a weight $\theta_j$ to each meta-path $\mathcal{P}_j$, and the overall
cohesiveness is given by the weighted average:
\begin{equation}
\Upsilon_{G} = \sum_{j=1}^r \theta_j \Upsilon_{G_{\mathcal{P}_j}}.
\end{equation}
We assume that the weights $\theta_j$'s can be learned. 
Due to space limitation,
readers can refer to~\cite{DBLP:dblp_conf/ecir/LuoGWL14,DBLP:dblp_conf/sdm/WanOKH15,DBLP:dblp_conf/cikm/WanLKYGCH15} for some example methods for learning meta-path weights.

We computed the \chn\ values of the three HIN classification tasks. Table~\ref{table:chn} shows the results.
We see that  DBLP has a much higher \chn\ value ($\Upsilon_{\mathit{DBLP}}$ = 0.536) 
compared with Yago ($\Upsilon_{\mathit{Yago}}$ = 0.209) and Freebase ($\Upsilon_{\mathit{Freebase}}$ = 0.185).
Again, this is consistent with our analysis that the connectivity assumption is more valid 
with DBLP than with Yago or Freebase. 
In Table~\ref{table:chn}, we also show the \chn\ values of the TSSNs derived from various meta-paths. 
For example, 
for DBLP, the TSSN $G_{\mathit{APA}}$, derived from the meta-path APA, is much more cohesive than
those given by other meta-paths. 
The interpretation is that co-authorship (which is captured by the meta-path APA) 
occurs mostly between authors of the same area. 
On the other hand, the small \chn\ value of $G_{\mathit{APTPA}}$ indicates that
authors of different areas could share the same keywords in their papers. 
For Yago Movie and Freebase Movie,
the meta-paths MDM and MDMDM derive the most cohesive TSSNs. 
Yet, their \chn\ values are much smaller than that of APA,
suggesting that it is more difficult for \tc\ to achieve high accuracy in classifying movies.

%Interestingly, these observations are consistent with those given in~\cite{DBLP:dblp_conf/cikm/WanLKYGCH15},
%which reveal that APA, MDM, and MDMDM are effective meta-paths in
%classifying objects for the three classification tasks. 

\begin{table}
\centering
\caption{Cohesiveness of HIN classification tasks}
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|}  \hline
\multicolumn{7}{|c|}{DBLP: $\Upsilon_{\mathit{DBLP}}$ = 0.536} \\ \hline
$\mathcal{P}$ & APA & APAPA & APVPA & APTPA  & & \\ \hline
$\Upsilon_{G_\mathcal{P}}$ & $0.733$ & $0.483$ & $0.393$ & $0.016$ & & \\ \hline \hline
\multicolumn{7}{|c|}{Yago: $\Upsilon_{\mathit{Yago}}$ = 0.209} \\ \hline
$\mathcal{P}$ & MAM & MDM & MWM & MAMAM  & MDMDM & MWMWM  \\ \hline
$\Upsilon_{G_\mathcal{P}}$ & $0.106$ & $0.313$ & $0.262$ & $0.065$ & $0.303$ & $0.214$  \\ \hline \hline
\multicolumn{7}{|c|}{Freebase: $\Upsilon_{\mathit{Freebase}}$ = 0.185 } \\ \hline
$\mathcal{P}$ & MAM & MDM & MPM & MAMAM & MDMDM & MPMPM \\ \hline
$\Upsilon_{G_\mathcal{P}}$ & $0.107$ & $0.326$ & $0.174$ & $0.086$ & $0.346$ & $0.123$ \\ \hline
\end{tabular}
\label{table:chn}
\end{table}


%By meta paths, we can derive several topology shrinking sub-networks from an HIN. So it is natural to measure the clustering property of an HIN from that of derived sub-networks.
%
%\begin{definition}
%Given an HIN $G$ and $K$ meta paths, $K$ sub-networks can be induced, which share $N$ clusters $C_1$, $C_2$, $...$, $C_N$. Each cluster $C_i$ contains $b_i$ objects, $i = 1, 2, ..., N$. For an arbitrary cluster $C_i$, we use $\bm{\theta_i}$ = ($\theta_{i_1}$, $\theta_{i_2}, ..., \theta_{i_K})^\mathrm{T}$ to represent weights of $K$ sub-networks. Let $\bm{\Upsilon}$ = ($\bm{\Upsilon_{G_{\mathcal{P}_1}}}$, $\bm{\Upsilon_{G_{\mathcal{P}_2}}}$, ..., $\bm{\Upsilon_{G_{\mathcal{P}_K}}})^\mathrm{T}\in R^{K \times N}$, $\bm{\theta}$ = ($\bm{\theta_1}$, $\bm{\theta_2}$, ..., $\bm{\theta_N})\in R^{K\times N}$, then \emph{HIN cluster cohesiveness vector} is defined as
%\begin{equation}
%\bm{\Upsilon_G^\prime} = (\bm{\theta_1^\mathrm{T}}\bm{\Upsilon}[:,1], \bm{\theta_2^\mathrm{T}}\bm{\Upsilon}[:,2], ..., \bm{\theta_N^\mathrm{T}}\bm{\Upsilon}[:,N])^\mathrm{T}
%\end{equation}
%and \emph{HIN cohesiveness} is the weighted average for clusters:
%\begin{equation}
%\label{eq:HIN_cohesiveness}
%\Upsilon_G = \bm{\beta^\mathrm{T}}\bm{\Upsilon_G^\prime}
%\end{equation}
%where $\bm{\beta} = (\frac{b_1}{\sum_{i=1}^N b_i}, \frac{b_2}{\sum_{i=1}^N b_i}, ..., \frac{b_N}{\sum_{i=1}^N b_i})^\mathrm{T}$.
%\end{definition}

%\begin{table}
%\centering
%\scriptsize
%\caption{DBLP sub-network cohesiveness}
%\label{table:DBLP_cohesiveness}
%\begin{tabular}{|c|c|c|c|} \hline
% APA & APAPA & APVPA & APTPA \\ \hline
%$0.733$ & $0.483$ & $0.393$ & $0.016$\\ \hline
%\end{tabular}
%\centering
%\caption{Yago Movie sub-network cohesiveness}
%\label{table:yagomovie_cohesiveness}
%\begin{tabular}{|c|c|c|c|c|c|} \hline
% MAM & MDM & MWM & MAMAM & MDMDM & MWMWM\\ \hline
%$0.106$ & $0.313$ & $0.262$ & $0.065$ & $0.303$ & $0.214$\\ \hline
%\end{tabular}
%\centering
%\caption{Freebase Movie sub-network cohesiveness}
%\label{table:freebasemovie_cohesiveness}
%\begin{tabular}{|c|c|c|c|c|c|} \hline
% MAM & MDM & MPM & MAMAM & MDMDM & MPMPM\\ \hline
%$0.107$ & $0.326$ & $0.174$ & $0.086$ & $0.346$ & $0.123$\\ \hline
%\end{tabular}
%\centering
%\caption{HIN cohesiveness on three datasets}
%\label{table:hin_cohesiveness}
%\begin{tabular}{|c|c|c|c|} \hline
% DBLP & Yago Movie & Freebase Movie \\ \hline
%$0.536$ & $0.209$ & $0.185$ \\ \hline
%\end{tabular}
%\end{table}

%Based on meta path, \emph{cohesiveness} is a new measure to how cohesive an HIN is. Experimental results are shown in table \ref{table:hin_cohesiveness}. Obviously, DBLP has larger cohesiveness value than other two networks, so transductive classification performs better on it, which proves our assumption. Based on the above analysis, both NetClus and cohesiveness reflect DBLP has better clustering structure. Then we make a summary: 
%
%\textbf{Summary:} An HIN with better clustering structure will lead to better transductive classification.
%
%We also show cohesiveness value of each sub-network on three HINs in tables \ref{table:DBLP_cohesiveness}, \ref{table:yagomovie_cohesiveness} and \ref{table:freebasemovie_cohesiveness}. We notice that sub-networks induced by APA, MDM and MDMDM are more cohesive. It reflects these meta paths are more effective, which coincides with the conclusion in \cite{DBLP:dblp_conf/cikm/WanLKYGCH15}. 

%\textcolor{blue}{Ben: The following is to be removed:
%xxxxxxxxxxxxxx}
%
%Since sub-networks derived by APA, MDM and MDMDM have larger cohesiveness values, transductive classification should perform better on them. However, according to tables \ref{table:accuracy:dblp_subnetworks}, \ref{table:accuracy:yago_subnetworks} and \ref{table:accuracy:freebase_subnetworks}, we notice that transductive classification on sub-networks derived by APVPA, MAM and MAMAM greatly outperforms that on other sub-networks. For meta paths APA, MDM and MDMDM, even though their induced sub-networks have larger cohesiveness values, transductive classification works poorly, which can be explained by the conclusion in \cite{DBLP:dblp_conf/cikm/WanLKYGCH15} that the average percentage of reachable objects from a given object by a meta path, referring to \emph{reach}, is too small. Furthemore, we perform \emph{normalized cuts} \cite{DBLP:dblp_conf/cvpr/ShiM97} on each sub-network and use NMI to be the measure. Tables \ref{table:DBLP_nmi}, \ref{table:yagomovie_nmi} and \ref{table:freebasemovie_nmi} show the results. We observe that sub-network induced by APVPA is better clustered than sub-network corresponding to APA in DBLP. Also MDM and MDMDM are not always better than others. These observations further reflect the poor reach of meta paths APA, MDM and MDMDM.
%
%\begin{table}
%\centering
%\scriptsize
%\caption{NMI on sub-networks of DBLP}
%\label{table:DBLP_nmi}
%\begin{tabular}{|c|c|c|c|} \hline
% APA & APAPA & APVPA & APTPA \\ \hline
%$0.025$ & $0.010$ & $0.654$ & $0.067$\\ \hline
%\end{tabular}
%\centering
%\caption{NMI on sub-networks of Yago Movie}
%\label{table:yagomovie_nmi}
%\begin{tabular}{|c|c|c|c|c|c|} \hline
% MAM & MDM & MWM & MAMAM & MDMDM & MWMWM\\ \hline
%$0.010$ & $0.024$ & $0.004$ & $0.053$ & $0.019$ & $0.002$\\ \hline
%\end{tabular}
%\centering
%\caption{NMI on sub-networks of Freebase Movie}
%\label{table:freebasemovie_nmi}
%\begin{tabular}{|c|c|c|c|c|c|} \hline
% MAM & MDM & MPM & MAMAM & MDMDM & MPMPM\\ \hline
%$0.186$ & $0.005$ & $0.003$ & $0.214$ & $0.014$ & $0.009$\\ \hline
%\end{tabular}
%\end{table}
%
%\begin{table}
%\centering
%\tiny
%\caption{Classification accuracy on sub-networks in DBLP}
%\label{table:accuracy:dblp_subnetworks}
%\resizebox{\linewidth}{!}
%{
%%\hspace{-0.5cm}
%\begin{tabular}{|c|c|c|c|c|} \hline
% percent of & \multirow{2}{*}{APA} & \multirow{2}{*}{APAPA} & \multirow{2}{*}{APVPA} & \multirow{2}{*}{APTPA}\\ 
%labeled authors&&&&\\\hline
%$0.1\%$ & $33.0\%$ & $33.7\%$ & $81.7\%$ & $30.0\%$\\ \hline
%$0.2\%$ & $37.3\%$ & $38.1\%$ & $89.0\%$ & $31.7\%$\\ \hline
%$0.3\%$ & $39.6\%$ & $41.5\%$ & $89.8\%$ & $33.3\%$\\ \hline
%$0.4\%$ & $41.8\%$ & $42.7\%$ & $90.3\%$ & $34.4\%$\\ \hline
%$0.5\%$ & $42.8\%$ & $44.0\%$ & $91.1\%$ & $35.3\%$\\ \hline
%\end{tabular}
%}
%\caption{Classification accuracy on sub-networks in Yago Movie}
%\label{table:accuracy:yago_subnetworks}
%\resizebox{1.05\linewidth}{!}
%{
%%\hspace{-0.5cm}
%\begin{tabular}{|c|c|c|c|c|c|c|} \hline
% percent of & \multirow{2}{*}{MAM} & \multirow{2}{*}{MDM} & \multirow{2}{*}{MWM} & \multirow{2}{*}{MAMAM} & \multirow{2}{*}{MDMDM} & \multirow{2}{*}{MWMWM}\\ 
%labeled movies&&&&&&\\\hline
%$1\%$ & $35.9\%$ & $1.0\%$ & $2.4\%$ & $34.9\%$ & $1.0\%$ & $2.6\%$ \\ \hline
%$2\%$ & $39.1\%$ & $2.1\%$ & $4.6\%$ & $39.1\%$ & $2.0\%$ & $4.7\%$ \\ \hline
%$3\%$ & $40.6\%$ & $3.0\%$ & $6.2\%$ & $40.7\%$ & $3.1\%$ & $6.2\%$ \\ \hline
%$4\%$ & $40.8\%$ & $3.9\%$ & $7.6\%$ & $41.0\%$ & $3.9\%$ & $7.5\%$ \\ \hline
%$5\%$ & $41.5\%$ & $4.8\%$ & $8.8\%$ & $41.3\%$ & $4.8\%$ & $8.7\%$ \\ \hline
%\end{tabular}
%}
%\caption{Classification accuracy on sub-networks in Freebase Movie}
%\label{table:accuracy:freebase_subnetworks}
%\resizebox{1.05\linewidth}{!}
%{
%%\hspace{-0.5cm}
%\begin{tabular}{|c|c|c|c|c|c|c|} \hline
% percent of & \multirow{2}{*}{MAM} & \multirow{2}{*}{MDM} & \multirow{2}{*}{MPM} & \multirow{2}{*}{MAMAM} & \multirow{2}{*}{MDMDM} & \multirow{2}{*}{MPMWPM}\\ 
%labeled movies&&&&&&\\\hline
%$1\%$ & $63.5\%$ & $1.4\%$ & $9.2\%$ & $63.7\%$ & $1.2\%$ & $9.6\%$ \\ \hline
%$2\%$ & $64.0\%$ & $2.7\%$ & $10.8\%$ & $64.3\%$ & $2.7\%$ & $11.0\%$ \\ \hline
%$3\%$ & $64.5\%$ & $3.8\%$ & $12.3\%$ & $65.2\%$ & $3.8\%$ & $12.1\%$ \\ \hline
%$4\%$ & $65.1\%$ & $5.0\%$ & $13.1\%$ & $65.5\%$ & $5.0\%$ & $13.4\%$ \\ \hline
%$5\%$ & $65.7\%$ & $6.1\%$ & $14.1\%$ & $66.0\%$ & $6.1\%$ & $14.4\%$ \\ \hline
%\end{tabular}
%}
%\end{table}
%From table \ref{table:hin_cohesiveness}, we also find that the cohesiveness of Yago Movie is larger than that of Freebase Movie, but transductive classification performs better on Freebase Movie. Based on new observations, we conclude that cohesiveness is an important factor to transductive classification, but it is not the only one. Since \emph{reach} can affect transductive classification, we propose another assumption.
%
%\begin{assumption}
%For a heterogeneous information network, if objects to be classified are more connected, transductive classification will perform better.
%\end{assumption}
%
%\textcolor{blue}{xxxxxxxxxxx}

\subsection{Connectedness}
We say that an HIN is highly connected if objects of the same label exhibit {\it strong connectivity}.
With respect to \tc, this connectivity should facilitate label propagation from one object to another of the same class.
To illustrate the idea, consider Figure~\ref{figure:compactness}, which shows two object clusters ($\Circle$ and $\Box$) in
a structural connectivity graph.
We see that objects in the $\Box$ cluster are strongly connected in the sense that if
an object in the cluster (say $y_1$) is labeled, the label can be propagated effectively to all other objects in the same cluster.
The $\Circle$ cluster, on the other hand, is less connected. 
In particular, if we consider only the intra-cluster edges of the $\Circle$ cluster, the $\Circle$ objects form two isolated components.
If object $x_1$ in component 1 is labeled, the label cannot be propagated to the objects in component 2 (e.g., $x_2$)
without going through the $\Box$ cluster.
Label propagation among the $\Circle$ objects is thus less effective.

We measure the \cnn\ of a cluster $C$ by the number of disconnected components ($\mathit{NDC}(C)$) in $C$ 
if only intra-cluster edges are considered.
For example, in Figure~\ref{figure:compactness}, the NDC of the $\Circle$ cluster is 2, while that of the $\Box$ cluster is 1.
The larger $\mathit{NDC}(C)$ is, the less is the \cnn\ of cluster $C$.
We normalize this measure to [0,1] and define {\it cluster connectedness}, $\Psi_C$:

%We still divide objects to be classified into different clusters indicated by their labels. Intuitively, if objects within a cluster are connected, label propagation will be promoted. On the contrary, if objects within a cluster are scattered in many disconnected components, label propagation will be blocked between components, which hinders transductive classification. As shown in figure \ref{figure:compactness}, cluster in black contains three components and each component is fully connected. Suppose the label of object B in component 2 is known, but it cannot be directly propagated to components 1 and 3 without going through A. It is more likely that objects in components 1 and 3 to be influenced by A but not B.

\begin{figure}
    \centering
        \includegraphics[width = 0.5\linewidth]{figure/Q1_compactness_new.pdf}
        \caption{An example illustrating \cnn}
        \label{figure:compactness} %% label for entire figure
\end{figure}

%To measure the connectivity of an HIN, we still utilize meta paths to derive sub-networks which contain same clusters. Similar to cohesiveness, we first measure the connectivity of a cluster in a sub-network.

%\begin{definition}
%For any cluster $C$ with $b$ objects, $count(C)$ represents the number of components within it. Obviously, $1\leq count(C)\leq b$. If $count(C) = 1$, all the objects are connected. If $count(C) = b$, all the objects are isolated. Intuitively, the connectivity of a cluster is inversely proportional to $count$ value. In addition, when two clusters have the same $count > 1$, it is reasonable to consider the one with more objects is more compact. Therefore, \emph{cluster compactness} is defined to measure the connectivity of a cluster:
\begin{equation}
\label{eq:cluster_compactness}
\Psi_C=\left\{ \begin{array}{ll}
               1& \mbox{ when } \mathit{NDC}(C) = 1,\\
               1-\frac{\mathit{NDC}(C)}{b}& \mbox{ when } \mathit{NDC}(C) > 1,\\
              \end{array}
       \right.
\end{equation}
%\end{definition}
where $b$ is the number of objects in $C$.

If there are $k$ clusters $C_1, ..., C_k$, corresponding to  $k$ labels of a classification task, 
let $\bm{\Psi} = (\Psi_{C_1}, \Psi_{C_2}, ..., \Psi_{C_k})^\mathrm{T}$. 
We define the \cnn\ of an HIN $G$ as the weighted average of the cluster \cnn:
%\begin{definition}
%For a meta path $\mathcal{P}$ induced sub-network $G_{\mathcal{P}}$, suppose there are $N$ clusters $C_1, C_2, ..., C_N$. Each cluster $C_i$ contains $b_i$ objects, $i = 1, 2, ..., N$.
%Since $G_\mathcal{P}$ consists of $N$ clusters, then we have \emph{sub-network cluster compactness vector} $\bm{\Psi_{G_\mathcal{P}}^\prime} = (\Psi_{C_1}, \Psi_{C_2}, ..., \Psi_{C_N})^\mathrm{T}$. 
%And \emph{sub-network compactness} is the weighted average for clusters:
\begin{equation}
\Psi_G = \bm{\beta}\bm{\Psi},
\end{equation}
where $\bm{\beta} = (\frac{b_1}{\sum_{i=1}^k b_i}, \frac{b_2}{\sum_{i=1}^k b_i}, ..., \frac{b_k}{\sum_{i=1}^k b_i})$.
%\end{definition}

Similar to our discussion of \chn,
if we use meta-paths $\mathcal{P}_1, ..., \mathcal{P}_r$ in \tc, we evaluate 
 $\Psi_{G_{\mathcal{P}_j}}$ for each TSSN $G_{\mathcal{P}_j}$.
The overall
\cnn\ of an HIN $G$ is the weighted average:
\begin{equation}
\Psi_{G} = \sum_{j=1}^r \theta_j \Psi_{G_{\mathcal{P}_j}},
\end{equation}
where $\theta_j$'s are the meta-path weights.

Table~\ref{table:cnn} shows the \cnn\ values of our classification tasks. 
The \cnn\ of the TSSN derived from each meta-path considered is also shown.
From the table, we see that DBLP has a much higher \cnn\ value (0.942) compared with
Yago (0.393) and Freebase (0.584). 
This means that authors of the same area mostly form a single structurally connected component.
The label of one author can therefore be very effectively propagated to other authors of the same area via meta-paths. 
Comparing the four meta-paths used in DBLP, we see that the \cnn\ values of APVPA and APTPA are even higher than that of APA.
The interpretation is that authors of the same area tend to attend the same conferences and use similar keywords in their papers,
but they do not necessarily co-author with each other. 
For Yago Movie and Freebase Movie, we see that MAM and MAMAM give relatively high \cnn\ values,
indicating that movies of the same genre tend to be starred by the same actors. 
However, the two movie HINs are generally much less connected than DBLP. 

\begin{table}
\caption{Connectedness of HIN classification tasks}
\centering
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|}  \hline
\multicolumn{7}{|c|}{DBLP: $\Psi_{\mathit{DBLP}}$ = 0.942} \\ \hline
$\mathcal{P}$ & APA & APAPA & APVPA & APTPA  & & \\ \hline
$\Psi_{G_\mathcal{P}}$ & $0.899$ & $0.920$ & $1.0$ & $1.0$ & & \\ \hline \hline
\multicolumn{7}{|c|}{Yago: $\Psi_{\mathit{Yago}}$ = 0.393} \\ \hline
$\mathcal{P}$ & MAM & MDM & MWM & MAMAM  & MDMDM & MWMWM  \\ \hline
$\Psi_{G_\mathcal{P}}$ & $0.567$ & $0.253$ & $0.281$ & $0.690$ & $0.253$ & $0.285$  \\ \hline \hline
\multicolumn{7}{|c|}{Freebase: $\Psi_{\mathit{Freebase}}$ = 0.584 } \\ \hline
$\mathcal{P}$ & MAM & MDM & MPM & MAMAM & MDMDM & MPMPM \\ \hline
$\Psi_{G_\mathcal{P}}$ & $0.970$ & $0.282$ & $0.350$ & $0.992$ & $0.282$ & $0.382$ \\ \hline
\end{tabular}
\label{table:cnn}
\end{table}

Now, let us study how \chn\ and \cnn\ 
are correlated to classification accuracy. We apply \gm\ on the three classification tasks.
For each one,
we further obtain the accuracy when only one meta-path (and its derived TSSN) is used.
Table~\ref{table:acc} shows the results.
For example,  if \gm\ uses only the meta-path APA to derive 
the structural connectivity between objects in DBLP, the classification accuracy is 42.8\%;
If all four meta-paths are considered, then \gm\ achieves an accuracy of 89.3\%.
Note that for DBLP, the training set is much smaller (0.5\%) than that of Yago Movie and Freebase Movie (5\%).

\begin{table}
\caption{Accuracies of applying \gm\ to HINs}
\centering
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|}  \hline
\multicolumn{7}{|c|}{DBLP: 0.5\% labeled objects, classification accuracy = 89.3\%}  \\ \hline
$\mathcal{P}$ & APA & APAPA & APVPA & APTPA  & & \\ \hline
acc. &42.8\% &44.0\% & 91.1\% & 35.3\% & & \\ \hline \hline
\multicolumn{7}{|c|}{Yago: 5\% labeled objects, classification accuracy = 49.2\%}  \\ \hline
$\mathcal{P}$ & MAM & MDM & MWM & MAMAM  & MDMDM & MWMWM  \\ \hline
acc. & $41.5\%$ & $4.8\%$ & $8.8\%$ & $41.3\%$ & $4.8\%$ & $8.7\%$  \\ \hline \hline
\multicolumn{7}{|c|}{Freebase: 5\% labeled objects, classification accuracy = 65.4\%}  \\ \hline
$\mathcal{P}$ & MAM & MDM & MPM & MAMAM & MDMDM & MPMPM \\ \hline
acc. &  $65.7\%$ & $6.1\%$ & $14.1\%$ & $66.0\%$ & $6.1\%$ & $14.4\%$ \\ \hline
\end{tabular}
\label{table:acc}
\end{table}

From Tables~\ref{table:chn}, \ref{table:cnn}, \ref{table:acc}, we draw the following observations:

\noindent{\bf (1)} The \chn\ and \cnn\ of DBLP are both much higher than those of Yago and Freebase, and
the classification accuracy of DBLP (89.3\%) is also much higher than those of Yago (49.2\%) and Freebase (65.4\%).

\noindent{\bf (2)} For DBLP, the meta-path APVPA gives the highest accuracy (91.1\%). This is because its TSSN is the most
connected (1.0) and is reasonably cohesive (0.393, which is higher than any \chn\ values in Yago or Freebase).

\noindent{\bf (3)} The accuracy of the TSSN due to meta-path APTPA (35.3\%) is much lower than that of APVPA (91.1\%) although 
both of them are perfect in their \cnn\ scores (1.0). The reason is that the \chn\ value of APTPA is
extremely low (0.016). This indicates that, with APTPA, although a label propagates well among objects within the same
cluster (high \cnn), the label also propagates over to other clusters as well (very low \chn).

\noindent{\bf (4)} For Yago and Freebase, although MDM and MDMDM give relatively cohesive TSSNs ($\Upsilon$: 0.303-0.346)
among all meta-paths for the two tasks,
the TSSNs are highly disconnected ($\Psi$: 0.253-0.282).
This explains why the classification accuracies using only MDM or MDMDM are so poor (6.1\%).

From these observations, we can conclude that  \chn\ and \cnn\ are highly correlated with classification accuracy. 
Also, both factors are important to the successful application of \tcrs.



%\begin{definition}
%Given an HIN $G$ and $K$ meta paths, we first derive $K$ sub-networks which share $N$ clusters $C_1$, $C_2$, $...$, $C_N$. Each cluster $C_i$ contains $b_i$ objects, $i = 1, 2, ..., N$. For an arbitrary cluster $C_i$, we use $\bm{\theta_i} = (\theta_{i_1}, \theta_{i_2}, ..., \theta_{i_K})^\mathrm{T}$ to represent weights of $K$ sub-networks. Let $\bm{\Psi}$ = ($\bm{\Psi_{G_{\mathcal{P}_1}}}$, $\bm{\Psi_{G_{\mathcal{P}_2}}}$, ..., $\bm{\Psi_{G_{\mathcal{P}_K}}})^\mathrm{T}$$\in R^{K \times N}$, $\bm{\theta}$ = ($\bm{\theta_1}$, $\bm{\theta_2}$, ..., $\bm{\theta_N}$)$\in R^{K\times N}$, then \emph{HIN cluster compactness vector} is defined as
%\begin{equation}
%\bm{\Psi_G^\prime} = (\bm{\theta_1^\mathrm{T}}\bm{\Psi}[:,1], \bm{\theta_2^\mathrm{T}}\bm{\Psi}[:,2], ..., \bm{\theta_N^\mathrm{T}}\bm{\Psi}[:,N])^\mathrm{T}
%\end{equation}
%and \emph{HIN compactness} is the weighted average for clusters:
%\begin{equation}
%\label{eq:HIN_compactness}
%\Psi_G = \bm{\beta^\mathrm{T}}\bm{\Psi_G^\prime}
%\end{equation}
%where $\bm{\beta} = (\frac{b_1}{\sum_{i=1}^N b_i}, \frac{b_2}{\sum_{i=1}^N b_i}, ..., \frac{b_N}{\sum_{i=1}^N b_i})^\mathrm{T}$.
%\end{definition}

%\emph{Compactness} reflects how connected a network is. The experimental results are shown in tables \ref{table:DBLP_compactness}, \ref{table:yagomovie_compactness}, \ref{table:freebasemovie_compactness} and \ref{table:hin_compactness}. We observe that 
%\newline{\small $\bullet$} sub-networks derived by APVPA, MAM and MAMAM are more compact, thus transductive classification performs better on them.
%\newline{\small $\bullet$} For APTPA, even though the compactness is large, the cohesiveness is too small, which largely reduces classification accuracy.
%\newline{\small $\bullet$} DBLP has the largest compactness value, so transductive classification performs best on it.
%\newline{\small $\bullet$} Compactness of Freebase Movie is much larger than that of Yago Movie, which explains why transductive classification performs better in Freebase Movie.
%
%\begin{table}
%\centering
%\scriptsize
%\caption{DBLP sub-network compactness}
%\label{table:DBLP_compactness}
%\begin{tabular}{|c|c|c|c|} \hline
% APA & APAPA & APVPA & APTPA \\ \hline
%$0.899$ & $0.920$ & $1.0$ & $1.0$\\ \hline
%\end{tabular}
%\centering
%\caption{Yago Movie sub-network compactness}
%\label{table:yagomovie_compactness}
%\begin{tabular}{|c|c|c|c|c|c|} \hline
% MAM & MDM & MWM & MAMAM & MDMDM & MWMWM\\ \hline
%$0.567$ & $0.253$ & $0.281$ & $0.690$ & $0.253$ & $0.285$\\ \hline
%\end{tabular}
%\centering
%\caption{Freebase Movie sub-network compactness}
%\label{table:freebasemovie_compactness}
%\begin{tabular}{|c|c|c|c|c|c|} \hline
% MAM & MDM & MPM & MAMAM & MDMDM & MPMPM\\ \hline
%$0.970$ & $0.282$ & $0.350$ & $0.992$ & $0.282$ & $0.382$\\ \hline
%\end{tabular}
%\centering
%\caption{HIN compactness on three datasets}
%\label{table:hin_compactness}
%\begin{tabular}{|c|c|c|c|} \hline
% DBLP & Yago Movie & Freebase Movie \\ \hline
%$0.942$ & $0.393$ & $0.584$ \\ \hline
%\end{tabular}
%\end{table}
%
%These observations prove assumption 2 and we summarize:
%
%\textbf{Summary:} An HIN with compact connectivity will result in good performance of transductive classification. 
%
%\input{tex/question3.tex}












==> tex/definition.tex <==
\section{Definitions}
\label{sec:definition}
In this section we give a formal problem definition.
%Table~\ref{table:symbol} lists some of the symbols used in this paper.

\comment{
\begin{table}
\caption{Descriptions of symbols}
\centering
\scriptsize
%\scriptsize
\begin{tabular}{|c|l|}
    \hline
    {\bf Notation} & \multicolumn{1}{c|}{\bf Description} \\ \hline
    $G = (V, E)$ 	& An HIN $G$ with object set $V$ and link set $E$ \\ \hline
    $\mathcal{T}, T_i, m$	&$\mathcal{T} = \{T_1,T_2,...,T_m\}$, a set of $m$ object types\\ \hline
    $\mathcal{A}_i, \mathcal{A}$	&Attribute set $\mathcal{A}_i$ of object type $T_i$, $\mathcal{A} = \bigcup_{i=1}^m{\mathcal{A}_i}$\\ \hline
    $G_{\mathcal{A}} = (V, E, \mathcal{A})$ 	& An attributed HIN $G_{\mathcal{A}}$ with attribute set $\mathcal{A}$ \\ \hline
%    $x, e, T$	&An arbitrary object $x$, edge $e$, object type $T$\\ \hline
%    $x_{ij}$					&  The $j$-th type-$T_i$ object\\ \hline
    $\mathcal{X}_i, n_i$	& The set $\mathcal{X}_i$ of type $T_i$ objects, $|\mathcal{X}_i| = n_i$ \\ \hline
    $T_G = (\mathcal{T}, \mathcal{R})$		& Network schema of HIN $G$ \\ \hline
%    $n, n_i$ 				&   $|\mathcal{V}|, |\mathcal{X}_i|$ \\ \hline
    $p_{x_u\leadsto{x_v}} \vdash \mathcal{P}$ & $p_{x_u\leadsto{x_v}}$ is an instance of the meta-path $\mathcal{P}$ \\ \hline
%    $\mathcal{P}, \mathcal{PS}$ 	& Meta path $\mathcal{P}$, a set of meta paths $\mathcal{PS}$\\ \hline
    $G_{T_i,\mathcal{P}}$, $G_\mathcal{P}$			                 & TSSN of object type $T_i$ induced by meta-path $\mathcal{P}$\\ \hline
%    $\mathcal{L}$, $L(x)$					& Training set $\mathcal{L}$; $L(x)$ = label of object $x$ if $x \in \mathcal{L}$ \\ \hline
    $F_i$				                                            	& Type $T_i$ object attribute matrix $\in {\mathbb{R}^{n_i\times {|\mathcal{A}_i|}}}$ \\ \hline
    $\mathcal{M}$, $\mathcal{C}$					& Must-link set and cannot-link set \\ \hline
    $\mathfrak{C} = \{C_1, ..., C_k\}$			                 	& A set of $k$ disjoint clusters  \\ \hline
   % $\Upsilon_{C}$, $\Upsilon_{G_\mathcal{P}}$, $\Upsilon_G$	& Cohesiveness of a cluster, a sub-network and an HIN\\ \hline
   % $\Psi_{C}$, $\Psi_{G_\mathcal{P}}$, $\Psi_G$	& Compactness of a cluster, a sub-network and an HIN\\ \hline
   
%    $\Upsilon_{C}$, $\Upsilon_{G_\mathcal{P}}$, $\Upsilon_G$	& Cohesiveness of a cluster, a sub-network and an HIN\\ \hline
%    $\Psi_{C}$, $\Psi_{G_\mathcal{P}}$, $\Psi_G$	& Compactness of a cluster, a sub-network and an HIN\\ \hline
%    $Q(\mathcal{P})$					& The proportion of qualified objects for meta path $\mathcal{P}$ \\ \hline
%    $E(\mathcal{P})$					& The effectiveness of meta path $\mathcal{P}$ \\ \hline
%    $U(\mathcal{P})$					& The usefulness of meta path $\mathcal{P}$ \\ \hline
%   
\end{tabular}
\label{table:symbol}
%\end{small}
\end{table}
}


\comment{
\begin{definition}
\textbf{Heterogeneous Information Network (HIN)}. Let $\cal{T}$ = $\{ t_1, \ldots, t_m \}$ be a set of $m$ object types.
Let $\cal{V}$ be a set of  $n$ objects.
Each object $x \in \cal{V}$ has a unique type, denoted by $T(x)$.
We use $\mathcal{X}_h$ to denote the set of all objects of type $t_h$,
i.e., $\mathcal{X}_h = \{x \in \mathcal{V} \; | \; T(x) = t_h \}$
and $\mathcal{V} = \cup_{h=1}^{m} \mathcal{X}_h$.
Let $n_h = |\mathcal{X}_h|$.
Let $\mathcal{E}$ be a set of links, which represents a binary relation between objects in $\mathcal{V}$.
An object $x_i$ is related to another object $x_j$ iff $(x_i, x_j) \in \mathcal{E}$.
An HIN $\mathcal{G} = \langle \mathcal{V}, \mathcal{E} \rangle$
is a set of objects $\mathcal{V}$ and a set of links $\mathcal{E}$.
\end{definition}
}

\begin{definition}
\label{def:ahin}
\textbf{Attributed Heterogeneous Information Network (AHIN)}. 
Let $\mathcal{T}$ = $\{T_1, ..., T_m \}$ be a set of $m$ object types.
For each type $T_i$, 
let $\mathcal{X}_i$ be the set of objects of type $T_i$
and $A_i$ be the set of attributes defined for objects of type $T_i$.
An object $x_j$ of type $T_i$ is associated with an attribute vector
$\bm f_{j} = (f_{j1}, f_{j2}, ..., f_{j|A_i|})$.
%For each type $T_i$, 
%let $n_i$ and $\mathcal{X}_i = \{ x_{i1}, ..., x_{in_i} \}$ be the number and the set of objects of type $T_i$, respectively.
An AHIN is a graph $G = (V, E, \mathcal{A})$, where
$V = \bigcup_{i=1}^m\mathcal{X}_i$ is a set of nodes,
$E$ is a set of links, each represents a binary relation between two objects in $V$,
and $\mathcal{A} = \bigcup_{i=1}^m{A_i}$.
If $m$ = 1 (i.e., there is only one object type), $G$ reduces to a homogeneous information network.
\hfill$\Box$
\end{definition}

%Given an HIN $G$, objects of type $T$ are usually attached with a set of \textbf{attributes} $A$
%and these attributes can be divided into different types.
%For example, restaurants in Yelp may have numerical attributes like the number of reviews, longitude and latitude, 
%ordinal attribute star level, boolean attribute reservation, etc.
%These attributes convey different information and may be useful in different clustering tasks.
%In this paper, we consider all these kinds of attributes.
%Including attributes to an HIN $G = (V, E)$, an \textbf{attributed heterogeneous information network (AHIN)} $G_{\mathcal{A}} = (V, E, \mathcal{A})$,
%where $\mathcal{A} = \bigcup_{i=1}^m{A_i}$.
%For each object $x_i$ of type $T$, the attribute vector is represented as $\bm f_{i} = (f_{i1}, f_{i2}, ..., f_{i|A|})$.

\begin{definition}
\textbf{Network schema}. A network schema is the meta template of
an AHIN $G = (V, E, \mathcal{A})$.
Let 
(1) $\phi: V \rightarrow \mathcal{T}$ be an object-type mapping that maps an object in $V$ into its type, and
(2) $\psi: E\rightarrow \mathcal{R}$ be a link-relation mapping that maps a link in $E$ into a relation in a set of 
relations $\mathcal{R}$.
The network schema of an AHIN $G$, denoted by $T_G = (\mathcal{T}, \mathcal{R})$,
shows how objects of different types are related by the relations in $\mathcal{R}$. 
$T_G$ can be represented by a {\it schematic graph} with $\mathcal{T}$ and $\mathcal{R}$ being the node set and the edge set, 
respectively.
Specifically, there is an edge ($T_i$, $T_j$) in the schematic graph iff there is a relation in $\mathcal{R}$ that relates
objects of type $T_i$ to objects of type $T_j$.
\hfill$\Box$
%
%
% with the object type mapping $\phi: V\rightarrow \mathcal{T}$ and the link mapping $\psi: E\rightarrow \mathcal{R}$, which is a directed graph defined over object types $\mathcal{T}$, with edges as relations from $\mathcal{R}$, denoted as $T_G = (\mathcal{T}, \mathcal{R})$.
\end{definition}

Figure~\ref{figure:subnetworks}(a) shows an example AHIN that models movie information 
(attribute information is not shown).
The AHIN consists of four object types: $\mathcal{T}$ = \{
movie ($\Diamond$), actor($\Box$), director($\Circle$), producer($\triangle$) \}.
There are also three relations in $\mathcal{R}$, which are illustrated by the three edges in the schematic
graph (Figure~\ref{figure:subnetworks}(b)). For example, the relation between {\it actor} and {\it movie} 
carries the information of which actor has acted in which movie.
Actors, directors and producers have attributes like age, gender, birthplace, while 
movies are associated with attributes like release date, box office, etc. 


\comment{
\begin{definition}
\textbf{Meta path}. A meta-path $\mathcal{P} = t_{i_1} \ldots t_{i_d}$ is a sequence of object types.
We use $\mathcal{P}[j]$ to denote the $j$-th object type ($t_{i_j}$) specified in the meta-path $\mathcal{P}$.
Given an HIN $G$ and a path $p$ in $G$,
let $|p|$ be the length (as measured by the number of objects) of path $p$ and $p[j]$ be the $j$-th object in $p$.
Path $p$
is an \emph{instance} of $\mathcal{P}$, denoted by $p \vdash \mathcal{P}$ iff
$p$ and $\mathcal{P}$ are of the same length and the types of the objects in $p$ match
those specified in $\mathcal{P}$. Formally,
$p \vdash \mathcal{P}$ iff
(1) $|p|$ = $d$ and
(2) $T(p[j]) = \mathcal{P}[j] \; \forall 1 \leq j \leq d$.
\end{definition}
}

\begin{definition}
\textbf{Meta-path}. A meta-path $\mathcal{P}$ is a path defined on the 
schematic graph of a network schema.
%$T_G = (\mathcal{T}, \mathcal{R})$.
A meta-path $\mathcal{P}$: $T_1\stackrel{R_1}{\longrightarrow} \cdots\stackrel{R_l}{\longrightarrow} T_{l+1}$
 defines a composite relation $R = R_1\circ \cdots \circ R_l$ 
 that relates objects of type $T_1$ to objects of type $T_{l+1}$.
 If two objects $x_u$ and $x_v$ are related by the composite relation $R$,
 then there is a path, denoted by $p_{x_u\leadsto{x_v}}$, that connects $x_u$ to $x_v$ in $G$.
 Moreover, the sequence of links in $p_{x_u\leadsto{x_v}}$ matches the sequence of relations
 $R_1$, ..., $R_l$ based on the link-relation mapping $\psi$.
 We say that $p_{x_u\leadsto{x_v}}$ is a {\it path instance} of $\mathcal{P}$, denoted by
 $p_{x_u\leadsto{x_v}} \vdash \mathcal{P}$.
 \hfill$\Box$
%  where $\circ$ denotes the composition operator on relations.
\end{definition}

As an example, the path $p_{M1 \leadsto M3} = M1\rightarrow A2 \rightarrow M3$
in Figure~\ref{figure:subnetworks}(a)
is an instance of  the meta-path Movie-Actor-Movie (abbrev. MAM). 
%
%
% has been applied to various data mining tasks including transductive classification, and it has been proved useful. Grempt utilizes meta paths where $T_1 = T_{l+1} $, and converts the original heterogeneous information network to several homogeneous \emph{topology shrinking sub-networks}.

%\begin{small}
\begin{figure}
    \centering
    \vspace{-3mm}
        \includegraphics[width = 0.9\linewidth]{figure/hin.pdf}
        \caption{{\scriptsize An AHIN (a) and its schematic graph (b)}}
        \label{figure:subnetworks}
        \vspace{-2mm}
\end{figure}
%\end{small}

\comment{
\begin{definition}
\textbf{Topology Shrinking Sub-network (TSSN)}. Given an HIN $G = (V, E)$, 
the TSSN of a certain object type $T_i$ derived from a meta-path $\mathcal{P}$
is a graph
whose nodes consist of only objects of type $T_i$ and whose edges connect objects that are related by
instances of $\mathcal{P}$. Formally,
the TSSN is the graph
 $G_{T_i,\mathcal{P}} = (\mathcal{X}_i, E_{T_i})$,
where 
$E_{T_i} = \{e_{uv} | p_{x_u\leadsto{x_v}} \vdash {\mathcal{P}}, x_u, x_v \in{\mathcal{X}_i}\}$.
We write $G_\mathcal{P}$ instead of $G_{T_i,\mathcal{P}}$ if the object type $T_i$ is implicitly known.
\hfill$\Box$
%
% can be denoted as $G_T = (V_T, E_T, R_T)$, $V_T = \mathcal{X}_T$, $E_T = \{e_{uv}|p_{x_u\leadsto{x_v}}\in{\mathcal{P}}, x_u, x_v \in{V_T}\}$ and $R_T = \{R_{uv}|R_{uv}$ is the weight of $e_{uv}\in{E_T}\}$, where $p_{x_u\leadsto{x_v}}$ denotes a path instance between $x_u$ and $x_v$.
\end{definition}

Figures \ref{figure:subnetworks}(c)-(e) show the TSSNs of type Movie derived from the meta-paths
MAM, MDM and MPM, respectively.
A TSSN shows how objects of a certain type are related by the composite relation given by a meta-path. 
For example, the meta-path MAM relates two movie objects if those movies share an actor. 
In Figure~\ref{figure:subnetworks}(c), movies M1 and M2 are connected by an edge in the TSSN because
actor A1 acted in both movies.
}

\begin{definition}
\label{def:user-guidance}
\textbf{Supervision constraint}.
The clustering process is supervised by a user through a constraint ($\mathcal{M}$, $\mathcal{C}$), where $\mathcal{M}$
and $\mathcal{C}$ are the {\it must-link set} and the {\it cannot-link set}, respectively. 
Each of these sets is a set of object pairs $(x_a, x_b)$.
An object pair in $\mathcal{M}$ represents that the two objects must belong to the same cluster,
while a pair in $\mathcal{C}$
indicates that the two objects  should not be put into the same cluster.
\hfill$\Box$
\end{definition}

\begin{definition}
\textbf{Semi-supervised clustering in an AHIN}.
\label{def:clustering}
Given an AHIN $G = (V,E,\mathcal{A})$, a supervision constraint ($\mathcal{M}$, $\mathcal{C}$),
a target object type $T_i$, the number of clusters $k$, and a set of meta-paths $\mathcal{PS}$,
the problem of semi-supervised clustering of type $T_i$ objects in $G$ is to
(1) discover an object similarity measure $S$ that is based on object attributes and meta-paths, and
(2) partition the objects in $\mathcal{X}_i$ into $k$ disjoint clusters $\mathfrak{C} = \{C_1, ..., C_k\}$
based on the similarity measure $S$ such that the clustering results best agree with the constraint 
($\mathcal{M}$, $\mathcal{C}$).
%\begin{itemize}\setlength{\itemsep}{-2pt}
%\item The object type $T$ to be clustered.
%\item The number of clusters $k$.
%\item A must-link set $\mathcal{M}$ and a cannot-link set $\mathcal{C}$.
%\item A set of meta paths $\mathcal{PS}$. 
%\end{itemize}
%and produces the following outputs:
%\begin{itemize}\setlength{\itemsep}{-2pt}
%\item A partitioning of the set $\mathcal{X}$  into $k$ disjoint clusters $\mathfrak{C} = \{C_1, ..., C_k\}$, where $\bigcup_{i=1}^k C_i = \mathcal{X}$ and
%$\bigcap_{i=1}^k C_i = \emptyset$.
%\item Meta path weight vector $\bm \lambda$, where $\lambda_i \geq 0$, $\sum_{i=1}^{|\mathcal{PS}|} \lambda_i = 1$.
%\item Attribute weight vector $\bm \omega$, where $\omega_i \geq 0$, $\sum_{i=1}^{|A|} \omega_i = 1$.
%\end{itemize}
\hfill$\Box$
\end{definition}


%\begin{example}
%Figure \ref{figure:subnetworks} shows topology shrinking sub-networks derived from an HIN by different meta paths. The network in the left is an movie related HIN composed of movies (M $\Diamond$), actors(A $\Box$), directors(D $\Circle$) and producers(P $\triangle$). By meta paths MAM, MDM and MPM, we can respectively derive homogeneous subnetworks (a), (b) and (c) for movies.
%\end{example}
%

%In this paper, we first investigate factors influencing the performance of transductive classification in HINs. Then based on the factors, we devise a black-box tester which can estimate the performance of transductive classification on a given HIN and thereby provide suggestions for users in whether choose transductive classification methods for a specific classification task.
%\begin{definition}
%\textbf{Black-box tester}. Given an HIN $G = (V, E)$, a specific classification task on objects of type $T_i$ with a set of labels ${LS}_i$, a set of meta paths $\mathcal{PS}$ and a training set of labeled objects $\mathcal{L}$, our objective is to provide a black-box tester which can judge the performance of transductive classification on $G$ and thereby guide users in choosing transductive classification. If the tester outputs \texttt{Yes}, it indicates good performance and strong recommendation. If the output is \texttt{No}, it represents poor performance and bad choice. In other cases, the tester will output \texttt{No idea and have a try}.
%\end{definition}




















==> tex/newcommand.tex <==
\newcommand{\bmx}{\bm{x}}
\newcommand{\dan}[1]{\textcolor{blue}{Dan:#1}}

==> tex/optimization.tex <==
\subsection{Model optimization}
\label{sec:optimization}

Our objective is to find the best clustering, or equivalently, the indicator vectors $\{\bm{z}_r\}_{r=1}^k$ that 
minimizes the penalty function $\mathcal{J}()$.
Note that $\mathcal{J}()$ is a function of $\bml$ and $\bmo$ (which are the weights of meta-paths and object
attributes), whose values need to be learned as well.
\schain\ learns these parameters using an iterative mutual update approach. 
Each iteration consists of two steps. First, given $\bml$ and $\bmo$, we find the optimal clustering 
$\{\bm{z}_r\}_{r=1}^k$. Second, given $\{\bm{z}_r\}_{r=1}^k$, we
find the optimal $\bml$ and $\bmo$.
\schain\ iterates until the change in the penalty is smaller than a threshold $\epsilon$ or 
a fixed number of iterations have been executed.
Next, we show how the two update steps are performed.

\subsubsection{Finding the optimal $\{${\boldmath $z$}$_r\}_{r=1}^k$ given {\boldmath $\lambda$} and \boldmath $\omega$}

For fixed values of $\bml$ and $\bmo$, $\mathcal{J}()$ is a function of $\bmz$.
We define a matrix $\tilde{Z}$, where its $r$-th column
$\tilde{Z}_{\cdot r}$ 
equals $D^{\frac{1}{2}}\bm{z}_r/(\bm{z}_r^TD\bm{z}_r)^{\frac{1}{2}}$. 
Note that since $\tilde{Z}^T\tilde{Z} = I_k$, where $I_k$ is the $k \times k$ identity matrix,
$\tilde{Z}$ is an orthonormal matrix.
For fixed values of $\bml$ and $\bmo$, minimizing $\mathcal{J}()$ is equivalent to minimizing:
%\begin{small}
\begin{equation}
\label{eq:obj:trans2}
\begin{split}
\mathcal{J}'(\tilde{Z}) & = \mathit{trace}(\tilde{Z}^TD^{-\frac{1}{2}}(D-S-W\circ S)D^{-\frac{1}{2}}\tilde{Z}), \\
%& = \mathit{trace}(\tilde{Z}^TD^{-\frac{1}{2}}DD^{-\frac{1}{2}}\tilde{Z}-\tilde{Z}^TD^{-\frac{1}{2}}(S+ W\circ S)D^{-\frac{1}{2}}\tilde{Z}) \\
& = \mathit{trace}(I_k-\tilde{Z}^TD^{-\frac{1}{2}}(S+W\circ S)D^{-\frac{1}{2}}\tilde{Z}).
\end{split}
\end{equation}
%\end{small}
Since $trace(I_k)$ is a constant, the above is equivalent to solving the following trace maximization problem:
\begin{equation}
\begin{split}
\label{eq:max}
& \max_{\tilde{Z}^T\tilde{Z} = I_k}\mathit{trace}(\tilde{Z}^TD^{-\frac{1}{2}}(S+W\circ S)D^{-\frac{1}{2}}\tilde{Z}).  \\
\end{split}
\end{equation}
Since $\tilde{Z}$ is a rigorous cluster indicator matrix, the optimization problem is NP-hard~\cite{DBLP:dblp_conf/icml/LongZWY06}.
To address this issue, we allow real relaxation to $\tilde{Z}$ so that its entries can assume real values. Then,
according to the Ky-Fan theorem~\cite{bhatia1997matrix}, 
the maximization problem (\ref{eq:max}) has a closed-form solution that corresponds to the subspace spanned 
by the top $k$ eigenvectors of $K = D^{-\frac{1}{2}}(S+W\circ S)D^{-\frac{1}{2}}$. 
Since $\tilde{Z}_{\cdot r} = D^{\frac{1}{2}}\bm{z}_r/(\bm{z}_r^TD\bm{z}_r)^{\frac{1}{2}}$,
we need to transform each $\tilde{Z}_{\cdot r}$ back to a real-relaxed $\bm z_r$. 
We first calculate
$U = D^{-\frac{1}{2}}\tilde{Z}$ and then
normalize it by column.
Each column in $U$ is a real-relaxed $\bm z_r$.
Finally, with the real relaxation, entries in $U$ take on fractional values, so the clustering is not
definite. To derive a hard clustering, 
we treat each row in $U$ as a feature vector of an object.
After row normalization on $U$, we adopt $k$-means to cluster objects.
%a postprocessing step is required and we adopt $k$-means to convert $\tilde{Z}$ to $\{\bm {z}_r\}_{r=1}^k$.
%we take the cluster membership values of each object (derivable from $\bmz$)
%as features of objects and cluster the objects using $k$-means based on these cluster membership features.

\subsubsection{Finding the optimal {\boldmath $\lambda$} and {\boldmath $\omega$} given $\{${\boldmath $z$}$_r\}_{r=1}^k$}
%After clusters are derived, they can be used to supervise the weight learning of meta paths and attributes, 
%because different meta paths and attributes play different roles in determining the formation of these clusters.
%Therefore, we can optimize $\bm \lambda$ and $\bm \omega$ based on the results of $\{\bm z_i\}_{i=1}^k$.

For fixed $\{\bm z_r\}_{r=1}^k$, $\mathcal{J}()$ is a function of $\bml$ and $\bmo$.
We rewrite Eq.~\ref{eq:obj:trans:reg} as:
\begin{small}
\begin{equation}
\label{eq:obj:trans3}
\begin{split}
\mathcal{J}(\bm \lambda, \bm \omega) & = 
%\sum_{i=1}^k\frac{\bm{z}_i^T(D-S- \mathcal{W} \circ S)\bm{z}_i}{\bm{z}_i^TD\bm{z}_i} + \gamma(||\bm\lambda||^2+||\bm \omega||^2) \\
%& = 
\sum_{r=1}^k\frac{\bm{z}_r^TD\bm{z}_r-\bm{z}_r^T(S+ \mathcal{W} \circ S)\bm{z}_r}{\bm{z}_r^TD\bm{z}_r} + \gamma(||\bm\lambda||^2+||\bm \omega||^2), \\
& = k - \sum_{r=1}^k\frac{\bm{z}_r^T(S+ \mathcal{W} \circ S)\bm{z}_r}{\bm{z}_r^TD\bm{z}_r} + \gamma(||\bm\lambda||^2+||\bm \omega||^2). \\
%& + \gamma(\|\bm \lambda\|^2 + \sum_{c=1}^k \|A_c\|_F^2),
\end{split}
\end{equation}
\end{small}
Since $k$ is a constant, minimizing $\mathcal{J}(\bml, \bmo)$ is equivalent to maximizing:
\begin{equation}
\label{eq:obj:trans4}
%\mathcal{J}''(\bml, \bmo) = 
\max_{\bm \lambda, \bm \omega} \sum_{r=1}^k\frac{\bm{z}_r^T(S+ \mathcal{W} \circ S)\bm{z}_r}{\bm{z}_r^TD\bm{z}_r}
- \gamma(||\bm \lambda||^2+||\bm \omega||^2).
\end{equation}
Note that the entries of matrices $S$ and $D$ are linear functions of $\bml$ and $\bmo$.
Therefore, the numerator and the denominator of each term in the summation are both linear functions of $\bml$ and $\bmo$.
Hence, (\ref{eq:obj:trans4})
can be rewritten as:
%can be reformulated to a nonlinear polynomial fractional programming (NPFP) problem~\cite{dinkelbach1967nonlinear}.

%\textbf{Nonlinear polynomial fractional programming problem (NPFPP)}.
%$f(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^p a_u\prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{b_u}\prod_{i=1}^k\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{c_{uij}}$, 
%$g(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^q r_u \prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{s_u}\prod_{i=1}^k\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{t_{uij}}$.
%Then Eq.~\ref{eq:obj:trans4} can be revised as
\begin{equation}
\label{eq:obj:trans5}
\mathcal{H}(\bml, \bmo) = \max_{\bm \lambda, \bm \omega} \frac{f(\bm \lambda, \bm \omega)}{g(\bm \lambda, \bm \omega)},
\end{equation}
where
$f(\bm \lambda, \bm \omega)$ and $g(\bm \lambda, \bm \omega)$ are two nonlinear multivariate polynomial functions.

It is shown in~\cite{dinkelbach1967nonlinear} that the maximization problem with the form shown in Eq.~\ref{eq:obj:trans5} can be solved by solving the following
related {\it non-linear parametric programming} problem:
%It is difficult to directly perform analysis on a NPFP problem to determine the existence of solution, so it is necessary to 
%convert this kind of problem into an easy-to-solve one. 
%
%\begin{theorem}
%\label{theo:NPFP}~\cite{DBLP:dblp_journals/jgo/TuyTK04}
%The above NPFP problem is equivalent to the following polynomial programming (PP) problem
%\begin{equation}
%\label{eq:obj:trans6}
%\max_{\bm \lambda, \bm \omega, \eta} \eta f(\bm \lambda, \bm\omega)
%\end{equation}
%subject to $\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$,$\lambda_i \geq 0$, $i = 1,2,...|\mathcal{PS}|$,
%$\sum_{j=1}^{|A|}\omega_j = 1$, $\omega_j \geq 0$, $j = 1,2,...|A|$
%and $0 \leq \eta \leq 1/g(\bm \lambda, \bm \omega)$.
%\comment{
%Proof: Suppose $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k, \hat \eta)$ is an optimal solution for Eq.~\ref{eq:obj:trans6},
%obviously, $\hat \eta = 1/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$ and $\hat \eta f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k) = 
%f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$. Then for any solution $(\bm \lambda, \{A_i\}_{i=1}^k)$ for NFPP,
%setting $\eta = 1/g(\bm \lambda, \{A_i\}_{i=1}^k)$ satisfies the constraints for PPPPC. Since $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k, \hat \eta)$
%corresponds to the maximum value of Eq.~\ref{eq:obj:trans6}, we have $\eta f(\bm \lambda, \{A_i\}_{i=1}^k) \leq \hat \eta f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$
%, i.e., 
%$f(\bm \lambda, \{A_i\}_{i=1}^k)/g(\bm \lambda, \{A_i\}_{i=1}^k) \leq$ $f(\hat{\bm \lambda},$ $\{\hat A_i\}_{i=1}^k)$$/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$.
%Therefore, $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$ solves NFPP.
%
%Conversely, suppose $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$ solves NFPP. Then for any solution $(\bm \lambda, \{A_i\}_{i=1}^k, \eta)$ for PPPPC, 
%we have $\eta f(\bm \lambda, \{A_i\}_{i=1}^k)$ $\leq f(\bm \lambda, \{A_i\}_{i=1}^k)/g(\bm \lambda, \{A_i\}_{i=1}^k) \leq f(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$. By setting $\hat \eta = 1/g(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k)$, obviously, $(\hat{\bm \lambda}, \{\hat A_i\}_{i=1}^k, \hat \eta)$ solves PPPPC.
%}
%\hfill$\Box$
%\end{theorem}
%
%According to Theorem~\ref{theo:NPFP}, the NPFP problem can be solved by 
%solving an equivalent PP problem at the cost of adding one more parameter.
%Obviously, the added parameter brings in new burden and is not preferred.
%Moreover, it is well known that the key to solving a global optimization problem is to transcend an incumbent value of the objective function,
%so we can reformulate the NPFP problem into a nonlinear parametric programming (NPP) problem and further simplify it.
%Using the same symbols in Eq.~\ref{eq:obj:trans5}, we define
\begin{definition}
\label{def:npp}
\textbf{[Non-linear parametric programming (NPP)]}
Let $f(\bml,\bmo)$ and $g(\bml,\bmo)$ be two multivariate polynomial functions. For a given $\mu$, find
\begin{equation}
\label{eq:obj:trans7}
F(\mu) = \max_{\bm \lambda, \bm \omega} \left( f(\bm \lambda, \bm \omega) - \mu g(\bm \lambda, \bm \omega) \right).
\end{equation}
In our context, the parameters $\bml$ and $\bmo$ are subject to the constraints listed at the end of Section~\ref{sec:penalty}.
%subject to $\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$,$\lambda_i \geq 0$, $i = 1,2,...|\mathcal{PS}|$ and
%$\sum_{j=1}^{|A|}\omega_j \newline= 1$, $\omega_j \geq 0$, $j = 1,2,...|A|$.
\hfill$\Box$
\end{definition}
In~\cite{dinkelbach1967nonlinear}, the following theorem is proved.
\begin{theorem}
\label{theorem2}
Given a fixed $\mu$, let $({\bm \lambda^*}, {\bm \omega^*})$ be the optimal solution to $F(\mu)$ (Eq.~\ref{eq:obj:trans7}).
$(\bm \lambda^*, \bm \omega^*)$ is also an optimal solution to $\mathcal{H}(\bml, \bmo)$ (Eq.~\ref{eq:obj:trans5}) if and only if $F(\mu) = 0$.
%$f(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^p a_u \prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{b_u}\prod_{i=1}^k$ $\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{c_{uij}}$, 
%$g(\bm \lambda, \{A_i\}_{i=1}^k) = \sum_{u=1}^q r_u \prod_{j = 1}^{|\mathcal{PS}|}(\lambda_j)^{s_u}\prod_{i=1}^k$ $\prod_{j=1}^{|\mathcal{A}|}((A_i)_{jj})^{t_{uij}}$.
\hfill$\Box$
\end{theorem}

Besides Theorem~\ref{theorem2}, a few lemmas are also proved in~\cite{dinkelbach1967nonlinear}:
%Theorem~\ref{theorem2} reduces the NPFP problem to a NPP problem \emph{in the same parameter space},
%which is much simpler compared with PP problem. Also it is much easier to solve a NPP problem than a NPFP problem.
%Besides, we have some lemmas to help with the optimization.

\begin{lemma}
\label{lemma1}
$F(\mu)$ is convex.
\comment{
Proof: Suppose $(\bm \lambda, \{A_i\}_{i=1}^k)$ is the solution corresponding to $\mu = t\mu_1 + (1-t)\mu_2$,
where $\mu_1 \neq \mu_2, 0 \leq t \leq 1$. Then we have $F(\mu) = f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu g(\bm \lambda, \{A_i\}_{i=1}^k)
= f(\bm \lambda, \{A_i\}_{i=1}^k) - (t\mu_1 + (1-t)\mu_2)g(\bm \lambda, \{A_i\}_{i=1}^k) = t(f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_1g(\bm \lambda, \{A_i\}_{i=1}^k))
+ (1-t)(f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_2g(\bm \lambda, \{A_i\}_{i=1}^k))$.
Obviously, $f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_1g(\bm \lambda, \{A_i\}_{i=1}^k) \leq F(\mu_1)$ and 
$f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_2g(\bm \lambda, \{A_i\}_{i=1}^k) \leq F(\mu_2)$,
which induces $F(t\mu_1 + (1-t)\mu_2) \leq tF(\mu_1)+(1-t)F(\mu_2)$.
}
\hfill$\Box$
\end{lemma}
\begin{lemma}
\label{lemma2}
$F(\mu)$ is continuous.
\hfill$\Box$
\end{lemma}
\begin{lemma}
\label{lemma3}
$F(\mu)$ is strictly monotonically decreasing, i.e., if $\mu_1 < \mu_2$, $F(\mu_1) > F(\mu_2)$.
\comment{
Proof: Suppose $(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k)$ is the solution corresponding to $\mu_2$. 
Then we have $F(\mu_2) = f(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) - \mu_2g(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) 
< f(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) - \mu_1g(\hat{\bm \lambda}, \{\hat{A}_i\}_{i=1}^k) \leq 
\max_{\bm \lambda, \{A_i\}_{i=1}^k} f(\bm \lambda, \{A_i\}_{i=1}^k) - \mu_1 g(\bm \lambda, \{A_i\}_{i=1}^k) = F(\mu_1)$
}
\hfill$\Box$
\end{lemma}
\begin{lemma}
\label{lemma4}
$F(\mu) = 0$ has a unique solution.
\hfill$\Box$
\end{lemma}
Due to space limit, 
readers are referred to~\cite{dinkelbach1967nonlinear, stancu2012fractional} for the proofs of the theorem and lemmas.

From Theorem~\ref{theorem2}, we need to find
a $\mu^*$ and its corresponding $({\bm \lambda^*}, {\bm \omega^*})$ such that $F(\mu^*) = 0$.
\schain\ does so by an iterative numerical method.
In each iteration, \schain\ computes a $\mu$ and $(\bml, \bmo)$.
Let $\mu_i$, $(\bml_i, \bmo_i)$ be those computed in the $i$-th iteration.
\schain\ first sets $\mu_1 = 0$ and in each iteration, performs two steps:
(Step 1:) Solve the NPP problem (Eq.~\ref{eq:obj:trans7}) for $\mu = \mu_i$ and set $(\bml_i, \bmo_i)$ to be the solution found. 
(Step 2:) Set $\mu_{i+1} = f(\bml_i, \bmo_i)/g(\bml_i, \bmo_i)$.
Next, we show theoretical properties of this update process.

\noindent{\bf Property 1:}
$\bm{F(\mu_1) > 0}$. 
Without loss of generality, we assume $f(\bml, \bmo) > 0$ and $g(\bml, \bmo) > 0$.\footnote{One can show that the quantity (\ref{eq:obj:trans4})
is bounded below by $-2\gamma$. We can add an arbitrary large constant to (\ref{eq:obj:trans4}) to make it, and thus 
$f(\bml, \bmo)$ and $g(\bml, \bmo)$, positive.}
Now, $F(\mu_1)$ = $F(0)$ = $\max_{\bml, \bmo} f(\bm \lambda, \bm \omega) > 0$.

\noindent{\bf Property 2: if} $\bm{F(\mu_i) > 0}$ {\bf then} 
$\bm {0 \leq F(\mu_{i+1}) < F(\mu_i)}$.
Since $(\bml_i, \bmo_i)$ is the solution of the NPP problem for $\mu = \mu_i$ (Eq. \ref{eq:obj:trans7}),
we have $f(\bml_i, \bmo_i) - \mu_i g(\bml_i, \bmo_i) = F(\mu_i) > 0$.
Hence, $\mu_{i+1} = f(\bml_i, \bmo_i)/g(\bml_i, \bmo_i) > \mu_i$.
By Lemma~\ref{lemma3}, $F(\mu_{i+1}) < F(\mu_i)$.
Also, we have
$F(\mu_{i+1})$ = $\max_{\bm \lambda, \bm \omega} ( f(\bm \lambda, \bm \omega) -\mu_{i+1}g(\bm \lambda, \bm \omega))
\geq f(\bm \lambda_i, \bm \omega_i) - \mu_{i+1} g(\bm \lambda_i, \bm \omega_i) = 0$.

From the properties, we see that \schain\ starts with a positive $F(\mu)$, whose value 
stays positive and decreases across iterations until it reaches 0.
The update procedure thus converges to the optimal values.
%The process is repeated until a certain maximum number of iterations have been executed, or until $F(\mu_i)$ becomes
%negative for some iteration $i$. 
%In the latter case, due to Lemma~\ref{lemma3}, we know that $\mu^* \in [\mu_{i-1}, \mu_i]$.
%\schain\ then switches to the bisection method:
%It computes $\mu_{i+1} = (\mu_{i-1} + \mu_i)/2$, and repeats either with the interval $[\mu_{i-1}, \mu_{i+1}]$ or $[\mu_{i+1}, \mu_i]$,
%depending on which interval contains $\mu^*$. 
The \schain\ algorithm is summarized in Algorithm~\ref{alg}.
\begin{algorithm}
\begin{small}
\caption{SCHAIN}
\label{alg}
\begin{algorithmic}[1]
%\Require $G=(V, E)$, $A$, meta-paths $\mathcal{P}$'s, $\mathcal{X}_i$, $\mathcal{L}$, $D$, $B$, $N_s$.
\Require $G$, $\mathcal{M}$, $\mathcal{C}$, $T_i$, $k$, $\mathcal{PS}$.
\Ensure $\mathfrak{C} = \{C_1, ..., C_k\}$
\State Compute similarity matrices $S_A$, $S_L$, and $S$
\State $t=0$, $\Delta \mathcal{J} = \infty$
%\State Derive $S$ by Eq.~\ref{eq:S}
\State $\bm \lambda = (\frac{1}{|\mathcal{PS}|}, ..., \frac{1}{|\mathcal{PS}|})$;
$\bm \omega = (\frac{1}{|A_i|}, ..., \frac{1}{|A_i|})$
%\State Calculate $\mathit{QS}(D)$
\While{$\Delta \mathcal{J} > \epsilon$ or $t$ < max\_iter}
%\State Construct $\mathcal{M}$ and $\mathcal{C}$
\LeftComment Step 1: Optimize $\{\bm z_r\}_{r=1}^k$ given {$\bm \lambda$} and $\bm \omega$
\State Solve Eq.~\ref{eq:max} to obtain real-relaxed $\tilde{Z}$
\State Calculate $U=D^{-1/2}\tilde{Z}$ and normalize it
\State Derive $\{{\bm z}_r\}_{r=1}^k$ from $U$ by k-means
\LeftComment Step 2: Optimize {$\bm \lambda$} and $\bm \omega$ given $\{${$\bm z$}$_r\}_{r=1}^k$
\State $j=1$; $\mu_j = 0$
%\For{$j = 0$ to $F(\mu)$ converges to 0}
\Repeat
\State Solve Eq.~\ref{eq:obj:trans7} with $\mu = \mu_j$ to obtain ${\bm \lambda}_{j}$, ${\bm \omega}_{j}$
\State $\mu_{j+1} = f({\bm \lambda}_{j}, {\bm \omega}_{j}) / g({\bm \lambda}_{j}, {\bm \omega}_{j})$; $j$++
\Until  $F(\mu_{j+1})$ converges to 0%($j$ > max\_iter2) %or ($F(\mu_j) < 0$) 
%\If{($F(\mu_j) < 0$)}
%\State use bisection method to determine $\bml$, $\bmo$
%\Else 
%\State $\bml = \bml_j$; $\bmo = \bmo_j$
%\EndIf
\State $\Delta \mathcal{J}$ = change in $\mathcal{J}$ with the updated $\{{\bm z_r}\}_{r=1}^k$, $\bml$, $\bmo$
\State $t$++
%\State $\bm \lambda^{t+1} = \hat{\bm \lambda}^{j+1}$; $\bm \omega^{t+1} = \hat{\bm \omega}^{j+1}$
\EndWhile
\State Decode $\{C_r\}_{r=1}^k$ from $\{{\bm z_r}\}_{r=1}^k$
\State \Return $\mathfrak{C} = \{C_1, ..., C_k\}$
\end{algorithmic}
\end{small}
\end{algorithm}






\comment{

In conclusion, to solve a NPFP problem, we need to first convert it into a NPP problem. 
To solve the NPP problem, it involves in two steps. The first step is to select a $\mu$ value and the second one is to solve the maximization problem in
Eq.~\ref{eq:obj:trans7} to get $(\bm \lambda, \bm \omega)$ and $F(\mu)$.
Since the final aim is to find the $\mu$ which makes $F(\mu) = 0$,
we adopt an iterative two-step update strategy to perform optimization.
Step 1: given a $\mu$, solve the maximization problem in Eq.~\ref{eq:obj:trans7} to get $(\bm \lambda, \bm \omega)$ and the $F(\mu)$ value.
Step 2: given $(\bm \lambda, \bm \omega)$, calculate a new $\mu$ value.
Due to the monotonically decreasing property of $F(\mu)$,
we can start from a $\mu$ which makes $F(\mu) > 0$. 
%and $F(0) = \max_{\bm \lambda, \bm \omega} f(\bm \lambda, \bm \omega) > 0$, 
%we can start from $\mu = 0$. 
After $(\bm \lambda, \bm \omega)$ is calculated, according to Proposition~\ref{prop1}, we assign $\mu = f(\bm \lambda, \bm \omega)/g(\bm \lambda, \bm \omega)$.
The iteration repeats until $F(\mu) = 0$.

Since $||\bm \lambda||^2 \leq 1$ and $||\bm \omega||^2 \leq 1$,
we usually add a term $2\gamma$ to the end of Eq.~\ref{eq:obj:trans4} 
to ensure $-\gamma(||\bm \lambda|| ^ 2 + ||\bm \omega||^2) + 2\gamma \geq 0$.
On the one hand, the added term is irrelevant to $\bm \lambda$ and $\bm \omega$,
so it will not influence the optimization result.
On the other hand, it can ensure the derived $f(\bm \lambda, \bm \omega) > 0$ in Eq.~\ref{eq:obj:trans5}.
Since $F(0) = \max f(\bm \lambda, \bm \omega) > 0$,
we can safely start from $\mu = 0$.


\begin{proposition}
\label{prop1}
Suppose $F(\hat \mu) > 0$ and $(\hat{\bm \lambda}, \hat{\bm \omega})$ solves Eq.~\ref{eq:obj:trans7} corresponding to $\hat \mu$, 
then $f(\hat{\bm \lambda}, \hat{\bm \omega})/g(\hat{\bm \lambda}, \hat{\bm \omega}) > \hat \mu$.

Proof: $F(\hat \mu) = \max_{\bm \lambda, \bm \omega} f(\bm \lambda, \bm \omega) - \hat \mu g(\bm \lambda, \bm \omega) =
f(\hat{\bm \lambda}, \hat{\bm \omega}) - \hat \mu g(\hat{\bm \lambda}, \hat{\bm \omega}) > 0$.
$g$ derives from Eq.~\ref{eq:obj:trans4}, as the denominator,
$g(\hat{\bm \lambda}, \hat{\bm \omega}) > 0$,
so we have $f(\hat{\bm \lambda}, \hat{\bm \omega})/g(\hat{\bm \lambda}, \hat{\bm \omega}) > \hat \mu$.
\hfill$\Box$
\end{proposition}

Based on the above iterative optimization method, the model will finally converge.
Proofs are listed as follows.
\begin{theorem}
\label{theorem3}
The proposed model finally converges.

Proof: The objective is to minimize Eq.~\ref{eq:obj:trans:reg}, which includes three parts.
First, $0 \leq \bm{z}_i^T(D-S)\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 1$.
Second, for $-(\bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i)$, we consider two extreme cases:
if all the object pairs in cluster $i$ are in the must-link set $\mathcal{M}$, then $0 \leq \bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 1$;
if all the object pairs in cluster $i$ are in the cannot-link set $\mathcal{C}$, then $-1 \leq \bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 0$,
so $-1 \leq \bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i \leq 1$, i.e., $-1 \leq -(\bm{z}_i^TW\circ S\bm{z}_i / \bm{z}_i^TD\bm{z}_i) \leq 1$.
Third, since $\gamma \geq 0$, $\gamma (||\bm \lambda||^2 + ||\bm \omega||^2)$ is convex, the constraints on $\bm \lambda$ and $\bm \omega$ are 
also convex, so  
%$\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$, $\sum_{i=1}^{|\mathcal{PS}|}\lambda_i = 1$,$\lambda_i \geq 0$ and $\lambda_j \geq 0$,
it must have a minimum value.
In conclusion, Eq.~\ref{eq:obj:trans:reg} has a lower bound.

Furthermore, the iterative optimization method, either optimizing $\{${\boldmath $z$}$_i\}_{i=1}^k$ or 
updating $\bm \lambda$ and $\bm \omega$, always decreases the objective function, so the convergence is guaranteed.
\hfill$\Box$
\end{theorem}

}








